On semi-invariants of filtered representations of quivers and the cotangent bundle of the enhanced Grothendieck-Springer resolution

We introduce the notion of filtered representations of quivers, which is related to usual quiver representations, but is a systematic generalization of conjugacy classes of $n\times n$ matrices to (block) upper triangular matrices up to conjugation by invertible (block) upper triangular matrices. With this notion in mind, we describe the ring of invariant polynomials for interesting families of quivers, namely, finite $ADE$-Dynkin quivers and affine type $\widetilde{A}$-Dynkin quivers. We then study their relation to an important and fundamental object in representation theory called the Grothendieck-Springer resolution, and we conclude by stating several conjectures, suggesting further research.

==> categories-correct-them-then-input.tex <==
  

 
 

\begin{theorem}\label{theorem:functorial-isomorphism} 
EDIT OR DELETE. 
Let $X$ be an indecomposable filtered representation of $Q$ 
such that all maps of the representation are strict exact. 
\begin{enumerate}
\item\label{item:functorial-isom-kernel} Suppose the vertex $i$ 
is a sink and all maps of the induced filtered representation $F_i^+X$ are strict exact. 
Then $F_i^+ \gr X= \gr F_i^+ X=0$ if and only if $X\cong L_i$. 
Otherwise, we have 
$\gr F_i^+ X \cong F_i^+ \gr X$ 
with  
\[  
\dim (\gr F_i^+ X)_i   
  = \sum_{\rho=(j\rightarrow i)} \dim \gr X_j - \dim \gr X_i,  
\]  
and $\gr F_i^- F_i^+ X \cong \gr X$.  
\item\label{item:functorial-isom-cokernel} Suppose the vertex $i$   
is a source and all maps of the induced filtered representation $F_i^- X$ are strict exact. 
Then $F_i^- \gr X = \gr F_i^- X=0$ if and only if $X\cong L_i$.  
Otherwise, we have 
$\gr F_i^- X \cong F_i^- \gr X$ 
with   
\[  
\dim (\gr F_i^- X)_i   
  = \sum_{\rho=(i\rightarrow j)} \dim \gr X_j - \dim \gr X_i,  
\]  
and $\gr F_i^+ F_i^- X \cong \gr X$. 
\end{enumerate}
\end{theorem} 





\begin{proof} 
We will first prove \eqref{item:functorial-isom-kernel}. 
If $X\cong L_i$, then $F_i^+ X=0$, the trivial representation. So $\gr F_i^+ X=0$. 
Moreover, $\gr X\cong X$ since the vector space at vertex $i$ is $\mathbb{C}^1$ and the vector space at all other vertices is $0$. 
So $F_i^+ \gr X=0$. 

Now suppose $F_i^+ \gr X = \gr F_i^+ X=0$. 
We will show $X\cong L_i$. 
Since $F_i^+$ does not change the vector space at $X_j$ for $j\not=i$, $X_j$ must have been $0$ for all $j\not=i$. 
Since $F_i^+X=0$, the vector space $X_i$ at $i\in Q_0$ is $\mathbb{C}^n$.  
Since $X$ is indecomposable, $X_i\cong \mathbb{C}$.  

Now suppose $X\not\cong L_i$ and consider  
\[   \bigoplus_{\rho = (j\rightarrow i)} X_j \stackrel{h}{\twoheadrightarrow} X_i\rightarrow 0; 
\] 
the map $h$ is surjective since $X$ is indecomposable. 
Applying the functor $F_i^+$ to $X$, we obtain the inclusion: 
\[ 
   X_j \leftarrow \ker h = X_i' = (F_i^+ X)_i, 
\] 
which has a natural factorization through 
\[ 
 \ker h \hookrightarrow \bigoplus_{\rho = (j\rightarrow i)} X_j \rightarrow  X_j. 
\] 
It is now clear that we have the short exact sequence 
\[ 
0 \rightarrow (F_i^+ X)_i \stackrel{\widetilde{h}}{\hookrightarrow} 
 \bigoplus_{\rho=(j\rightarrow i)} X_j  
 \stackrel{h}{\twoheadrightarrow} X_i \rightarrow 0.  
\]  
Since $X$ is indecomposable, $F_i^+ X$ is also an indecomposable representation. 
Next we apply $\Rees(-)$ to obtain 
\[ 
0 \rightarrow \Rees(F_i^+ X)_i \stackrel{\Rees(\widetilde{h})}{\hookrightarrow} 
 \bigoplus_{\rho=(j\rightarrow i)} \Rees(X_j)  
 \stackrel{\Rees(h)}{\twoheadrightarrow} \Rees(X_i) \rightarrow 0,   
\]  
which is still exact due to the following reasons:  
since $\Rees(X)$ is an indecomposable graded representation, $\Rees(h)$ is surjective, and  
since $\Rees(F_i^+ X)$ is a graded subrepresentation of $\Rees(X)$,  
$\Rees(F_i^+X)$ is indecomposable and $\Rees(\widetilde{h})$ is injective.  
Finally, apply the associated graded functor to see that the short exact sequence is still preserved: 
\[ 
0 \rightarrow \gr (F_i^+ X)_i 
  \hookrightarrow \bigoplus_{\rho=(j\rightarrow i)} \gr X_j 
\stackrel{\overline{h}}{\twoheadrightarrow} \gr X_i \rightarrow 0 
\] 
since all linear maps of $X$ and $F_i^+X$ are strict exact: 
      $\bigoplus_j X_j \twoheadrightarrow X_i$ is a part of the representation $X$  
			while  
			$(F_i^+ X)_i \hookrightarrow \bigoplus_j X_j$ is a part of the representation $F_i^+ X$. 


Now, applying the $\gr$ functor first, we have 
\[ 
0 \rightarrow \ker \overline{h} \hookrightarrow \bigoplus_{\rho=(j\rightarrow i)} \gr X_j 
\stackrel{\overline{h}}{\twoheadrightarrow} \gr X_i \rightarrow 0,  
\]  
where $\overline{h}$ is surjective since all linear maps of $X$ are strict exact, and 
$\ker \overline{h}$ is naturally an inclusion. 
Applying $F_i^+$ to $\gr X$, 
the associated graded vector space at vertex $i$ has been replaced with  
\[ 
\gr X_j \leftarrow  (F_i^+ \gr X)_i. 
\] 
Since the reflection functor doesn't change vector spaces at vertices $j$ different from $i$, we have 
\[ 
0 \rightarrow (F_i^+ \gr X)_i \hookrightarrow \bigoplus_{\rho=(j\rightarrow i)} \gr X_j
\stackrel{\overline{h}}{\twoheadrightarrow} \gr X_i \rightarrow 0, 
\] 
with $(F_i^+ \gr X)_i=\ker \overline{h}$ by definition of $F_i^+$, 
which maps injectively into $\bigoplus_{\rho=(j\rightarrow i)} \gr X_j$. 
By the Five Lemma, 
$(F_i^+ \gr X)_i \cong \gr (F_i^+ X)_i$, and the dimension relation follows immediately. 
Finally,  
   we have $F_i^- F_i^+ X \cong X$ since  
   $(F_i^- F_i^+ X)_j = X_j$ for $j\not=i$ and 
   $(F_i^- F_i^+ X)_i = \coker \widetilde{h} = \im h= X_i$. 
   Thus, $\gr F_i^- F_i^+ X$ with the induced filtration is isomorphic to $\gr X$. 




Next, we will prove \eqref{item:functorial-isom-cokernel}. 
Suppose $X\cong L_i$ and $i$ is a source. 
Then $\gr X = X$ and since $(F_i^- \gr X)_i=\coker(\mathbb{C}\rightarrow \oplus 0)=0$ and $(F_i^- \gr X)_j=0$  
for all $j\not=i$,  
$F_i^- \gr X=0$. 
Similarly, since $F_i^- X$ is the zero representation, 
$\gr F_i^- X=0$. 

Now suppose $F_i^- \gr X=\gr F_i^- X=0$.
Since $(F_i^- X)_j= X_j$ for all $j\not=i$, 
$\gr(F_i^- X)_j=0$ for $j\not=i$ implies $X_j=0$ for $j\not=i$. 
Since $\gr (F_i^-X)_i=0$ by assumption, $(F_i^-X)_i=0$. 
So $X_i \cong \mathbb{C}^n$. 
Since $X$ is indecomposable, $X_i\cong \mathbb{C}$. 


Thus, assume $X \not\cong L_i$. 
Let $X$ be a filtered representation satisfying above assumptions and consider $DX=X^{op}$, 
where $X^{op}$ is the indecomposable representation obtained from the opposite quiver 
$Q^{op}=(Q_0,Q_1^{op})$,  
where all arrows of $Q^{op}$ are in reverse orientation than of the arrows of $Q$.  
In $X^{op}$, we have $X_i\rightarrow \bigoplus_{i\rightarrow j} X_j$. 
Since $X^{op}$ is indecomposable, $X_i\stackrel{k}{\hookrightarrow}\bigoplus_{i\rightarrow j} X_j$ is injective. 
We apply the reflection functor $F_i^-$ to obtain $X_j\twoheadrightarrow \coker k$, which factors through as the composition of an inclusion and a projection: 
\[ 
X_j \rightarrow \bigoplus_{i\rightarrow j} X_j \twoheadrightarrow \coker k. 
\] 
Thus the short exact sequence is obtained: 
\[ 
0\rightarrow X_i \stackrel{k}{\hookrightarrow} \bigoplus_{i\rightarrow j} X_j \stackrel{\widetilde{k}}{\twoheadrightarrow} \coker k\rightarrow 0,  
\]  
where $(F_i^-(X^{op}))_i=\coker k$. 
Next, we still have a short exact sequence when the associated graded functor is applied: 
\[ 
0\rightarrow \gr X_i \stackrel{k}{\hookrightarrow} \bigoplus_{i\rightarrow j} \gr X_j \twoheadrightarrow \gr \coker k \rightarrow 0  
\] since $X^{op}$ and $F_i^-(X^{op})$ are strict exact. 


Now apply $\gr$ first to get 
\[ 
0 \rightarrow \gr X_i \stackrel{\overline{k}}{\hookrightarrow}\bigoplus_{i\rightarrow j} \gr X_j,
\]  
which is still injective because maps of $X^{op}$ are strict exact. 
Next we apply $F_i^-$ to get 
\[ 
\gr X_j \twoheadrightarrow \coker \overline{k}=(F_i^- \gr X^{op})_i, 
\] 
which factors through 
\[  
\gr X_j \rightarrow \bigoplus_{i\rightarrow j} \gr X_j \twoheadrightarrow \coker \overline{k}. 
\]  
So again, a short exact sequence is obtained: 
\[ 
0 \rightarrow \gr X_i \stackrel{\overline{k}}{\hookrightarrow} \bigoplus_{i\rightarrow j}\gr X_j \twoheadrightarrow \coker \overline{k}\rightarrow 0.
\] 
By the Five Lemma, $\gr(F_i^- X^{op} )_i\cong (F_i^-\gr X^{op})_i$ implies 
$\gr F_i^-X^{op} \cong F_i^- \gr X^{op}$ and the dimension relation. 

Finally, we have $F_i^+ F_i^- X^{op}\cong X^{op}$ since 
\[  
(F_i^+ F_i^- X^{op})_j \cong X_j^{op} \mbox{ for } j\not=i
\]  
and $(F_i^+ F_i^- X^{op})_i=\ker \widetilde{k}= \im k\cong X_i \cong X_i^{op}$
since $k$ is injective. 
Thus, 
$\gr F_i^+ F_i^- X^{op} \cong \gr X^{op}$ as claimed. 
\end{proof} 

 
Let $D:F^{\bullet}Rep(Q,\beta) \rightarrow F^{\bullet}Rep(Q^{op}, \beta)$ be the functor that  takes $X$ to $X^{op}$.  
Classically, we have $F_i^-\circ D = D\circ F_i^+$.  
Under what conditions do we have  
$\gr F_i^- \circ D = D \circ \gr F_i^+$?  
Should we assume that $X$ is strict exact?  
\[ 
\xymatrix@-1pc{ 
F^{\bullet} Rep(Q,\beta) \ar[rrrr]^D \ar[dd]_{F_i^+} & & & & F^{\bullet} Rep(Q^{op},\beta) \ar[dd]^{F_i^-} \\ 
& & \circlearrowleft & & \\ 
F^{\bullet}Rep(F_i^+Q,F_i^+\beta) \ar[rrrr]^D & & & & F^{\bullet}Rep((F_i^+Q)^{op}, F_i^+\beta)
                                              = F^{\bullet}Rep(F_i^-Q^{op},F_i^-\beta). \\ 
}
\] 

 

 

\begin{lemma}\label{lemma:functorial-isomorphism} 
EDIT OR DELETE.  
Let $X,Y,Z\in F^{\bullet} Rep(Q,\beta)$ be representations such that all linear maps associated to an arrow of the quiver are block diagonals. 
Suppose $0\rightarrow X \rightarrow Y \rightarrow Z$ is a strict exact sequence. 
Then we have natural functorial isomorphisms 
$F_i^+(\gr X) \cong \gr F_i^+ (X)$, 
$F_i^+(\gr Y) \cong \gr F_i^+ (Y)$, and 
$F_i^+(\gr Z) \cong \gr F_i^+ (Z)$. 
Similarly, 
suppose $ X \rightarrow Y \rightarrow Z\rightarrow 0$ is a strict exact sequence. 
Then we have natural functorial isomorphisms 
$F_i^-(\gr X) \cong \gr F_i^- (X)$, 
$F_i^-(\gr Y) \cong \gr F_i^- (Y)$, and 
$F_i^-(\gr Z) \cong \gr F_i^- (Z)$. 
\end{lemma}



\begin{proof} 


\end{proof} 





\begin{lemma}\label{lemma:reflection-functor-gr-SES}
\mbox{}
EDIT OR DELETE.  
\begin{enumerate}
\item  Let $0 \rightarrow X\rightarrow Y \rightarrow Z$ be a strict exact sequence of filtered representations of a quiver. Let $i\in Q_0$ be a sink. Then 
$0 \rightarrow F_i^+ \gr X\rightarrow F_i^+ \gr Y \rightarrow F_i^+ \gr Z$ 
is left exact. 
\item Let $X\rightarrow Y\rightarrow Z\rightarrow 0$ be a strict exact sequence of filtered representations of a quiver. Let $i\in Q_0$ be a source. Then 
$F_i^-\gr X \rightarrow F_i^-\gr Y \rightarrow F_i^- \gr Z\rightarrow 0$ is right exact. 
\end{enumerate} 
\end{lemma}




 
\begin{proof}
Let $0 \rightarrow X\rightarrow Y \rightarrow Z$  
be a strict exact sequence of filtered representations of a quiver and suppose 
$i\in Q_0$ is a sink. 
This implies that 
$0\rightarrow \gr X \rightarrow \gr Y \rightarrow \gr Z $ is exact. 
Since $F_i^+$ is a left exact functor,  
$0\rightarrow F_i^+ \gr X \rightarrow F_i^+ \gr Y \rightarrow F_i^+ \gr Z$ is left exact. 


 
Now suppose $X\rightarrow Y\rightarrow Z\rightarrow 0$ is a strict exact sequence of filtered representations of a quiver and suppose $i\in Q_0$ is a source.   
Then $\gr X\rightarrow \gr Y\rightarrow \gr Z\rightarrow 0$ is exact. 
Since $F_i^-$ is a right exact functor, 
$F_i^- \gr X\rightarrow F_i^- \gr Y\rightarrow F_i^- \gr Z\rightarrow 0$ is right exact. 
\end{proof}











 
\begin{lemma}\label{lemma:gr-reflection-representations} 
\mbox{}  
EDIT OR DELETE.   
\begin{enumerate} 
\item\label{item:gr-reflection-representations-sink} Let 
$0\rightarrow X \rightarrow Y \rightarrow Z$ be a strict exact sequence of filtered representations of a quiver, where the maps are filtered maps. 
Let $i\in Q_0$ be a sink. Then 
$0\rightarrow \gr F_i^+ X \rightarrow \gr F_i^+  Y \rightarrow \gr F_i^+  Z$ is left exact. 
\item\label{item:gr-reflection-representations-source} Let 
$X\rightarrow Y \rightarrow Z\rightarrow 0$ 
be a strict exact sequence of filtered representations of a quiver, 
where the maps are filtered maps. 
Let $i\in Q_0$ be a source. Then 
$ \gr F_i^- X \rightarrow \gr F_i^-  Y \rightarrow \gr F_i^-  Z\rightarrow 0$ is right exact.  
\end{enumerate}
\end{lemma}


\begin{proof} 


\end{proof}



 
\begin{lemma}\label{lemma:graded-reflection-functors} 
EDIT OR DELETE.  
The reflection functors $F_i^+$ and $F_i^-$ are left and right exact, respectively, 
for strict exact sequence of filtered representations. 
\end{lemma} 

\begin{proof} 

\end{proof}















==> generalizing-gs-resolution.tex <==
 

\chapter{Generalizing the Grothendieck-Springer resolution} 

We generalize $\widetilde{\mathfrak{g}}\twoheadrightarrow \mathfrak{g}$ 
to quiver varieties. 
 
 


We extend the classical result in \cite{MR2838836} that $\widetilde{\mathfrak{g}}\stackrel{\pi}{\twoheadrightarrow} \mathfrak{g}$ 
is generically finite and dominant (projective) of degree $|W|$ to quiver varieties. 
The projective morphism $\pi$ is a symplectic resolution which factors through 
$\widetilde{\mathfrak{g}}\rightarrow \mathfrak{g}\times_{\mathfrak{h}/W}\mathfrak{h}\rightarrow \mathfrak{g}$, i.e., $\widetilde{\mathfrak{g}}=\{(x,\mathfrak{b})\in \mathfrak{g}\times G/B:x\in\mathfrak{b} \}$ is smooth. 



\section{Background}\label{section:background-generalizing-gs-resolution-to-quiver-vars} 
%\subsection{Background}\label{subsection:background-generalizing-gs-resolution-to-quiver-vars}

Let $B$ act on $G\times \mathfrak{b}$ via $b.(Q,x)=(Qb^{-1},bxb^{-1})$. 
Let $\widetilde{\mathfrak{g}}=G\times_B \mathfrak{b}=G\times \mathfrak{b}/B\subseteq G\times \mathfrak{b}$ be the space of all $B$-orbits on $G\times \mathfrak{b}$. 

Let $\phi:G\times_B \mathfrak{b}\rightarrow \{(x,\mathfrak{b})\in \mathfrak{g}\times G/B:x\in \mathfrak{b} \}$ be the map 
$\phi:(Q,x)\mapsto (QxQ^{-1}, QB/B)$, which is an isomorphism of projective schemes.  
Consider the projections 
$\widetilde{\mathfrak{g}}\stackrel{\pi_1}{\longrightarrow}\mathfrak{g}$ and 
$\widetilde{\mathfrak{g}}\stackrel{\pi_2}{\longrightarrow}G/B$. 
Since the preimage of $\mathfrak{b}$ via $\pi_2$ is $\mathfrak{b}$, $\pi_2$ is a vector bundle over $G/B$. 
Next, consider $\pi_1:G\times_B \mathfrak{b}\rightarrow \mathfrak{g}$, where 
$\pi_1:(Q,x)\mapsto QxQ^{-1}$. 
The projection $\pi_1$ onto the first factor is closed and a proper surjection since $G/B$ is compact and $\mathfrak{g}$ is the union of all Borel subalgebras of $\mathfrak{g}$. 
Over regular elements % such elements have centralizer whose dimension is as small as possible 
of $\mathfrak{g}$,  it is finite-to-one of degree $|W|$. 





==> section-affine-quotient-of-GS-resolution-invariants.tex <==
 

 

 
 
 

 



The locus $\mu_B^{-1}(0)$ is $B$-invariant since 
for $f$ vanishing on $\mu_B^{-1}(0)$ and for $b\in B$, 
$b.f$ vanishes on $b.\mu_B^{-1}(0)$. 
Since $\mu_B$ is $B$-equivariant, $b.\mu_B^{-1}(0)=\mu_B^{-1}(0)$. 
So $b.f$ vanishes on $\mu_B^{-1}(0)$, which implies the ideal $I(\mu_B^{-1}(0))$ is $B$-invariant. 
Thus, although the ideal is $B$-invariant, each generator of $I(\mu_B^{-1}(0))$ may not be $B$-invariant,  
which the following example shows. 

Let $n=2$. Then 
\[ 
\mu_B(r,s,i,j)=\left[ 
\begin{array}{cc}  
r_{12}s_{21}+x_1y_1 & * \\ 
(r_{22}-r_{11})s_{21} +x_2 y_1 & -r_{12}s_{21}+x_2 y_2 \\ 
\end{array}\right] \in \mathfrak{b}^*,  
\] 
and 
$I(\mu_B^{-1}(0))=\langle r_{12}s_{21}+x_1y_1,-r_{12}s_{21}+x_2 y_2, (r_{22}-r_{11})s_{21} +x_2 y_1  \rangle$. 
Since 
\[ 
\begin{aligned} 
brb^{-1}= 
\left[ \begin{array}{cc} 
r_{11} 	& \dfrac{b_{12}}{b_{22}} (r_{22}-r_{11})+\dfrac{b_{11}}{b_{22}} r_{12} \\  
0 			& r_{22} \\ 
\end{array} 
\right], 
&\hspace{4mm}
bsb^{-1} = 
\left[ \begin{array}{cc} 
s_{11}+\dfrac{b_{12}}{b_{11}} s_{21} & * \\ 
\dfrac{b_{22}}{b_{11}} s_{21} & s_{22} - \dfrac{b_{12}}{b_{11}} s_{21} \\ 
\end{array} 
\right],   \\ 
bi = \left[ \begin{array}{c} 
b_{11}x_1 + b_{12}x_2 \\ 
b_{22} x_2 \\ 
\end{array}\right],  
&\hspace{4mm}
jb^{-1} =   
\left[ 
\begin{array}{cc}  
\dfrac{y_1}{b_{11}} & \dfrac{y_2}{b_{22}}-\dfrac{b_{12}}{b_{11}b_{22}} y_1 \\  
\end{array}\right],    \\ 
\end{aligned} 
\] 
the generators of the ideal under the $B$-action will then become 
\[ 
\begin{aligned} 
r_{12}s_{21}+x_1y_1    &\mapsto  \left( \dfrac{b_{12}}{b_{22}} (r_{22}-r_{11})+\dfrac{b_{11}}{b_{22}} r_{12}\right)\left(\dfrac{b_{22}}{b_{11}} s_{21}\right) 
+ (b_{11}x_1 + b_{12}x_2)\left(\dfrac{y_1}{b_{11}} \right)  \\ 
	&\hspace{4mm}= (r_{12} s_{21} + x_1 y_1) + \dfrac{b_{12}}{b_{11}} ((r_{22} - r_{11}) s_{21} + x_2 y_1) \\ 
-r_{12}s_{21}+x_2 y_2  &\mapsto  -\left( \dfrac{b_{12}}{b_{22}} (r_{22}-r_{11})+\dfrac{b_{11}}{b_{22}} r_{12}\right)\left(\dfrac{b_{22}}{b_{11}} s_{21}\right) 
+ (b_{22}x_2)\left( \dfrac{y_2}{b_{22}}-\dfrac{b_{12}}{b_{11}b_{22}} y_1 \right)  \\ 
	&\hspace{4mm}= (-r_{12} s_{21} + x_2 y_2) - \dfrac{b_{12}}{b_{11}} ((r_{22} - r_{11}) s_{21} + x_2 y_1) \\ 
(r_{22}-r_{11})s_{21} +x_2 y_1 &\mapsto 
					(r_{22} - r_{11})\left(\dfrac{b_{22}}{b_{11}} s_{21}\right) + (b_{22} x_2)\left(\dfrac{y_1}{b_{11}}\right) =  \dfrac{b_{22}}{b_{11}}((r_{22}-r_{11})s_{21} +x_2 y_1).  \\ 
\end{aligned} 
\]  
In the next Chapter, we restrict to the regular semi-simple locus of $\mu_B$, i.e., this locus consists of pairwise 
distinct eigenvalues $r_{\iota\iota}$ of the matrix $r\in \mathfrak{b}$. 
Thus we can rewrite the off-diagonal generator of the ideal $I(\mu_B^{-1}(0))$ as $s_{21}=-x_2y_1/(r_{22}-r_{11})$. 
We then replace all occurrences of $s_{21}$ in the other two ideal generators using this relation to obtain 
\[ 
\begin{aligned} 
\mathbb{C}[\mu_B^{-1}(0)^{rss}] 
&= \dfrac{\mathbb{C}[T^*(\mathfrak{b}\times \mathbb{C}^2)][(r_{11}-r_{22})^{-1}]}{
\left\langle x_1 y_1 -r_{12} \left( \dfrac{x_2y_1}{r_{22}-r_{11}} \right),
x_2 y_2 + r_{12}\left( \dfrac{x_2y_1}{r_{22}-r_{11}}  \right), 
s_{21} + \dfrac{x_2y_1}{r_{22}-r_{11}}  
\right\rangle 
}   \\ 
&\cong \dfrac{\mathbb{C}[T^*(\mathfrak{b}\times \mathbb{C}^2)][\widehat{s}_{21}][(r_{11}-r_{22})^{-1}]}{
\left\langle x_1 y_1 -r_{12} \left( \dfrac{x_2y_1}{r_{22}-r_{11}} \right),
x_2 y_2 + r_{12}\left( \dfrac{x_2y_1}{r_{22}-r_{11}}  \right)    
\right\rangle 
} \hspace{4mm} \mbox{ where } \widehat{s}_{21}\mbox{ denotes that we omit }s_{21}.    \\ 
\end{aligned} 
\] 
We will soon see that 
\[ 
\begin{aligned} 
\mathbb{C}[\mu_B^{-1}(0)^{rss}]^B 
&= \dfrac{\mathbb{C}\left[ 
r_{11},r_{22},s_{11}',s_{22}', x_1 y_1 -r_{12} \left( \dfrac{x_2y_1}{r_{22}-r_{11}} \right),
x_2 y_2 + r_{12}\left( \dfrac{x_2y_1}{r_{22}-r_{11}}  \right)  
\right][(r_{11}-r_{22})^{-1}]}{
\left\langle x_1 y_1 -r_{12} \left( \dfrac{x_2y_1}{r_{22}-r_{11}} \right),
x_2 y_2 + r_{12}\left( \dfrac{x_2y_1}{r_{22}-r_{11}}  \right)    
\right\rangle 
}  \\ 
&\cong \mathbb{C}[\mathbb{C}^4 \setminus \Delta_2] = \mathbb{C}[\mathbb{C}^4]_{r_{11}-r_{22}}. 
\end{aligned} 
\] 
Thus, here in the $rss$-locus, 
we note that we were able to re-write the ideal generators in such a way so that each generator is a $B$-invariant function. 


Firstly, it is clear that the diagonal entries $r_{11}$ and $r_{22}$ are $B$-invariant, and $\Tr(s)= s_{11}+s_{22}$ is also a $B$-invariant polynomial from previous lemmas.  
Next, we recall $T^*(\mathfrak{b}\times \mathbb{C}^2)$: 
\[ 
\xymatrix@-1pc{ 
\mathrel{\substack{W(1)\\ \circ\\ \mathbb{C}^1}} \ar@/^/[rr]^{i} & & 
\mathrel{\substack{W(2)\\ \bullet \\ \mathbb{C}^2 }}\ar@/^/[ll]^j \ar@(r,d)[]^{s}  \ar@(r,u)[]_{r}, 
} 
\] 
where the vector space assigned to vertex $1$ is $W(1)=\mathbb{C}^1$ and the vector space assigned to vertex $2$ is $W(2)=\mathbb{C}^2$. 
Using the technique from --,  
we obtain the following invariants. 
Consider 
\[ \mathbb{C}^2 \oplus \mathbb{C}^2 \longrightarrow \mathbb{C}^2\oplus \mathbb{C}^2 
\] 
with the map given as a matrix of representations of paths: 
\[  
\left[ \begin{array}{cc} 
t_1 ij & t_2 \Inoindex_2 \\ 
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array} 
\right],  
\]   
where $t_i$'s are formal variables, $\Inoindex_2$ is a $2\times 2$ matrix, and $ij$ is a general representation of a path obtained by following $j$ then $i$. 
The determinant of this matrix is given as 
\[ 
\det\left[ 
\begin{array}{cc} 
t_1 ij & t_2 \Inoindex_2 \\  
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array} 
\right]  
=  
\det\left[ 
\begin{array}{cccc} 
t_1 (x_1 y_1) & t_1 (x_1 y_2) & t_2 & 0 	\\  
t_1 (x_2 y_1) & t_1 (x_2 y_2) & 0 	& t_2 \\  
		t_3  			& 			0 			& t_4 & 0 	\\  
			0 	 		& 		t_3 			& 0 	& t_4 \\   
\end{array} \right] = t_2^2 t_3^2 - (x_1 y_1 + x_2 y_2)t_1t_2t_3 t_4. 
\] 
We see that $x_1 y_1+x_2 y_2$ is an invariant polynomial since for   
\[   
f_{(r,s,i,j)}(t_1,t_2,t_3,t_4) = 
\det
\left[ 
\begin{array}{cc}  
t_1 ij & t_2 \Inoindex_2 \\  
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array}  
\right],    
\]  
\[ 
\begin{aligned} 
b.f_{(r,s,i,j)}(t_1,t_2,t_3,t_4) 
&= 
\det
\left[ 
\begin{array}{cc}  
t_1 (b^{-1}i)(jb ) & t_2 \Inoindex_2 \\  
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array}  
\right] \\ 
&= 
\det
\left[ 
\begin{array}{cc}  
b^{-1}(t_1 ij)b 					& b^{-1}(t_2 \Inoindex_2)b \\  
b^{-1}(t_3 \Inoindex_2)b 	& b^{-1}(t_4 \Inoindex_2)b \\ 
\end{array}  
\right] \\ 
&= 
\det \left( 
\left[ \begin{array}{cc} b^{-1} & 0 \\ 0 & b^{-1} \\ \end{array}\right] 
\left[ 
\begin{array}{cc}  
t_1 i j  & t_2 \Inoindex_2 \\  
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array}  
\right]
\left[ \begin{array}{cc} b & 0 \\ 0 & b \\ \end{array}\right]  
\right) \\ 
&= \det
\left[ 
\begin{array}{cc}  
t_1 i j  & t_2 \Inoindex_2 \\  
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array}  
\right]  \\ 
&= f_{(r,s,i,j)}(t_1,t_2,t_3,t_4).   \\ 
\end{aligned}  
\]   
Now consider 
\[ \mathbb{C}^2 \oplus \mathbb{C}^2 \longrightarrow \mathbb{C}^2 \oplus \mathbb{C}^2,   
\] 
where  
\[ 
\det
\left[ 
\begin{array}{cc}   
t_1 s 					& t_2 \Inoindex_2 \\ 
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array} 
\right] = 
\det\left[ 
\begin{array}{cccc} 
t_1 s_{11} & t_1 * 			& t_2 & 0  	\\  
t_1 s_{21} & t_1 s_{22} & 0 	& t_2  \\ 
		t_3 	 & 		0 			& t_4 & 0  		\\ 
		0 		 & 		t_3 		&	 0 	& t_4  \\ 
\end{array} 
\right]   = t_2^2 t_3^2 - (s_{11} + s_{22}) t_1 t_2 t_3 t_4 + (s_{11} s_{22} - * s_{21}) t_1^2 t_4^2. 
\]  
   Since a polynomial containing the equivalent class $*$ is not well-defined, we obtain just one invariant polynomial 
   $s_{11}+s_{22}$. 
Consider 
\[
 \mathbb{C}^2 \oplus \mathbb{C}^2 \longrightarrow \mathbb{C}^2 \oplus \mathbb{C}^2, 
\]  
where  
\[  \begin{aligned} 
\det\left[  
\begin{array}{cc}  
t_1 (r-r_{22}\Inoindex_2 )s & t_2\Inoindex_2 \\ 
t_3 \Inoindex_2 & t_4 \Inoindex_2 \\ 
\end{array}  
\right]  &= 
\det\left[ 
\begin{array}{cccc} 
t_1 ((r_{11} - r_{22}) s_{11} + r_{12} s_{21})& t_1((r_{11} - r_{22}) s_{12} + r_{12} s_{22}) & t_2 & 0 \\ 
 0  &  0  & 0 & t_2 \\ 
t_3 & 0   & t_4 & 0 \\ 
 0  & t_3 & 0 & t_4 \\   
\end{array} 
\right]   \\ 
&=  t_2^2 t_3^2 - ((r_{11}-r_{22}) s_{11} + r_{12} s_{21}) t_1 t_2 t_3 t_4. \\
\end{aligned} 
\]  
 One can check that $(r_{11}-r_{22}) s_{11} + r_{12} s_{21}$ is a $B$-invariant polynomial. 
Next, consider 
\[ \mathbb{C}^2 \oplus \mathbb{C}^2 \longrightarrow \mathbb{C}^2 \oplus \mathbb{C}^2,  
\] 
where 
\[ 
\begin{aligned}
\det\left[ 
\begin{array}{cc} 
t_1 (r-r_{11}\Inoindex_2)s & t_2 \Inoindex_2 \\ 
t_3 \Inoindex_2  & t_4 \Inoindex_2 \\ 
\end{array} 
\right]  
&= 
\det\left[ \begin{array}{cccc} 
t_1 (r_{12} s_{21}) 						& t_1 (r_{12} s_{22}) & t_2 & 0 \\ 
t_1 ((r_{22} - r_{11} ) s_{21}) & t_1 ((r_{22} - r_{11}) s_{22}) & 0 & t_2 \\ 
							t_3 							&  0  & t_4 & 0 \\ 
  							0 							& t_3 & 0 & t_4 \\  
\end{array} 
\right]  \\
&= t_2^2 t_3^2 + ((r_{11} - r_{22}) s_{22} - r_{12} s_{21}) t_1 t_2 t_3 t_4. \\ 
\end{aligned}
\] 
Then $(r_{11} - r_{22}) s_{22} - r_{12} s_{21}$ is also an invariant polynomial. 
Next consider 
\[ 
\mathbb{C}^2\longrightarrow \mathbb{C}^2, 
\] 
where the determinant of this map is 
\[ 
\begin{aligned}
\det\left[ 
\begin{array}{cc} 
t_1 s 						& t_2 \Inoindex_2 \\
t_3 \Inoindex_2  	& t_4 r \\ 
\end{array} 
\right] 
&= 
\det\left[ 
\begin{array}{cccc} 
t_1 s_{11}& t_1 *      & t_2 				& 0 \\
t_1 s_{21}& t_1 s_{22} & 0 					& t_2 \\ 
		t_3 	& 		 0 	 	 & t_4 r_{11} & t_4 r_{12} \\ 
		0			& 		t_3 	 & 0 					& t_4 r_{22}\\ 
\end{array} 
\right] \\ 
&= t_2^2 t_3^2 
- (r_{11} s_{11} + r_{22} s_{22} + r_{12} s_{21}) t_1 t_2 t_3 t_4 
+ (r_{11} r_{22} (s_{11} s_{22} - * s_{21})) t_1^2 t_4^2. \\ 
\end{aligned}
\]  
Here, we obtain just one invariant polynomial 
$r_{11} s_{11} + r_{22} s_{22} + r_{12} s_{21}$. 
Finally, consider 
\[ \mathbb{C}^2 \oplus \mathbb{C}^2 \longrightarrow \mathbb{C}^2 \oplus \mathbb{C}^2,  
\] 
where the determinant of this map is 
\[ 
\begin{aligned} 
\det\left[ 
\begin{array}{cc} 
t_1 s & t_2 \Inoindex_2 \\ 
t_3 r & t_4 \Inoindex_2 \\ 
\end{array}\right] 
&=  
\det\left[ 
\begin{array}{cccc} 
t_1 s_{11}& t_1 *     & t_2 & 0  \\ 
t_1 s_{21}& t_1 s_{22}&  0  & t_2 \\ 
t_3 r_{11}& t_3 r_{12}& t_4 & 0 \\
     0    & t_3 r_{22}&  0  & t_4 \\
\end{array} 
\right]   \\ 
&= (r_{11} r_{22}) t_2^2 t_3^2 
- (r_{11} s_{22} + r_{22} s_{11} - r_{12} s_{21}) t_1 t_2 t_3 t_4 + (s_{11} s_{22} - * s_{21}) t_1^2 t_4^2. \\ 
\end{aligned}
\] 
The polynomial $r_{11}r_{22}$ is a $B$-invariant polynomial, which is a product of the invariant polynomials $r_{11}$ and $r_{22}$. 
Thus, $r_{11} s_{22} + r_{22} s_{11} - r_{12} s_{21}$ is the only $B$-invariant generator that we will take into account. 
We have found other invariant polynomials by varying the size of the matrices and quiver paths 
but these (other $B$-invariant) polynomials vanish mod the ideal, which is the main reason why we didn't list them. 


In summary, we have found the following $B$-invariant generators on $T^*(\mathfrak{b}\times \mathbb{C}^2)$: 
\begin{itemize}
\item $r_{11}$ 
\item $r_{22}$ 
\item $s_{11}+s_{22} = \Tr(s)$
\item $x_1y_1+x_2y_2 = \Tr(ij)$
\item $f = (r_{11}-r_{22})s_{11} +r_{12}s_{21}$
\item $g = (r_{11}-r_{22})s_{22}-r_{12}s_{21}$
\item $h = r_{11}s_{11}+r_{22}s_{22}+r_{12}s_{21}$
\item $k = r_{11}s_{22}+r_{22}s_{11}-r_{12}s_{21}$.   
\end{itemize} 
Recall that on the locus where $r_{11}-r_{22}$  is nonvanishing, 
we can divide $f$ and $g$ by $r_{11}-r_{22}$. Then $s_{11}'= f/(r_{11}-r_{22})$ and $s_{22}' = g/(r_{11}-r_{22})$, where 
$s_{11}'$ and $s_{22}'$ are the diagonal coordinates of $s\in \mathfrak{b}^*$ 
after when they have been diagonalized by a certain $b\in B$.  Thus,  
$f$ and $g$ written out as rational functions are given in the chapter for the $rss$-locus. 
\[   
\begin{aligned}  
\mathbb{C}[\mu_B^{-1}(0)] = \dfrac{\mathbb{C}[T^*(\mathfrak{b}\times \mathbb{C}^2)]}{
I(\mu_B^{-1}(0))}  
&= \dfrac{\mathbb{C}[T^*(\mathfrak{b}\times \mathbb{C}^2)]}{
\langle r_{12}s_{21}+x_1 y_1, -r_{12}s_{21}+x_2 y_2, (r_{22}-r_{11})s_{21}+x_2 y_1\rangle} \\ 
&=  \dfrac{\mathbb{C}[T^*(\mathfrak{b}\times \mathbb{C}^2)]}{
\langle r_{12}s_{21}+x_1 y_1, x_1y_1 + x_2 y_2, (r_{22}-r_{11})s_{21}+x_2 y_1\rangle}. \\ 
\end{aligned} 
\] 
Now, calculating the coordinate ring of the affine quotient $\mu_B^{-1}(0)/\!\!/B$, 
\[ 
\begin{aligned}
\mathbb{C}[\mu_B^{-1}(0)]^B 
&=  \mathbb{C}[\overline{r_{11}},\overline{r_{22}},\overline{s_{11}+s_{22}},\overline{x_1y_1+x_2y_2}, \overline{f},\overline{g},\overline{h},\overline{k}] \hspace{4mm}\mbox{ where }\overline{f}:=f\mod I(\mu_B^{-1}(0)) \\ 
&= \mathbb{C}[\overline{r_{11}},\overline{r_{22}},\overline{s_{11}+s_{22}}, 
\overline{f},\overline{g},\overline{h},\overline{k}]  \hspace{4mm} \mbox{ since } x_1y_1+x_2y_2\in  I(\mu_B^{-1}(0)) \\ 
&= \mathbb{C}[\overline{r_{11}},\overline{r_{22}},\overline{s_{11}+s_{22}}, \overline{f},\overline{g},\overline{h}]  \hspace{4mm} \mbox{ since } \overline{f}-\overline{g}-\overline{h}+\overline{k} = 0 \\ 
&= \mathbb{C}[\overline{r_{11}},\overline{r_{22}},\overline{s_{11}+s_{22}}, \overline{f},\overline{g}]  \hspace{4mm} 
\mbox{ since } \overline{g}-\overline{r_{11}}(\overline{s_{11}}+\overline{s_{22}})+\overline{h} = 0 \\ 
&= \dfrac{\mathbb{C}[R_1,R_2,T,S_1,S_2]}{
\langle 
R_1 S_1 + R_1 S_2 + R_1 R_2 T - R_1^2 T  
\rangle 
} 
= \dfrac{\mathbb{C}[R_1,R_2,T,S_1,S_2]}{
\langle R_1 (S_1 + S_2 + (R_2 - R_1) T) \rangle 
} 
 \\ 
\end{aligned}
\] 
 

Remark~\ref{remark:hilbert-scheme-of-n-points-symmetric-product} is given so that we can compare the affine quotients 
$\mu_B^{-1}(0)/\!\!/B$ and $\mu_G^{-1}(0)/\!\!/G$. 

\begin{remark}\label{remark:hilbert-scheme-of-n-points-symmetric-product} 
In the construction of the Hilbert scheme of $n$ points on a complex plane, recall the moment map: 
\[ \mu_G:T^*(\mathfrak{gl}_n \times \mathbb{C}^n)\longrightarrow \mathfrak{g}^*, \hspace{4mm} \mu_G:(r,s,i,j)\mapsto [r,s]+ij. 
\] 
Then for $n=2$, using coordinates $\mathbb{C}[\mathbb{C}^2 \times \mathbb{C}^2]=\mathbb{C}[r_{11},r_{22},s_{11},s_{22}]$, 
we have 
$\mu_G^{-1}(0)/\!\!/G\cong S^2\mathbb{C}^2$, with 
\[ \begin{aligned} 
\mathbb{C}[S^2\mathbb{C}^2] &= \mathbb{C}[\mathbb{C}^2\times \mathbb{C}^2/S_2] \\ 
&=\mathbb{C}[\mathbb{C}^2\times \mathbb{C}^2]^{S_2} \\ 
&=\mathbb{C}[r_{11}+r_{22}, s_{11}+s_{22}, r_{11}^2+r_{22}^2, s_{11}^2+s_{22}^2, 
r_{11}s_{11}+r_{22}s_{22}] \\ 
&= \dfrac{\mathbb{C}[R_1,S_1,R_2,S_2,T]}{
\langle  
-2T^2+2R_1S_1T+2R_2S_2-S_2R_1^2-R_2S_1^2 
\rangle.  
}  
\end{aligned}  
\] 
So $S^2\mathbb{C}^2$ is a singular $4$ dimensional variety sitting in $\mathbb{C}^5$. 
Furthermore, there is a notion of symmetry between the $r_{\iota\iota}$'s and $s_{\iota\iota}$'s. 
\end{remark} 


Next, we will analyze the singular locus of $\mu_B^{-1}(0)/\!\!/B$ 
by locating where all the partials of 
$\phi$ vanish, where  
$\phi=  R_1 S_1 + R_1 S_2 + R_1 R_2 T - R_1^2 T$. 
So 
\begin{itemize} 
\item $\phi_{R_1} = S_1+S_2+R_2T - 2 R_1 T$ 
\item $\phi_{R_2} = R_1 T$
\item $\phi_T 		= R_1 (R_2 -R_1)$
\item $\phi_{S_1} = R_1$
\item $\phi_{S_2} = R_1$
\end{itemize} 
imply the singular locus of the affine quotient consists of the points where 
$R_1=0$ and $S_1 + S_2 + R_2 T = 0$. 


Need to interpret the above! 










 

==> section-construction-of-filtered-quiver-vars.tex <==

\chapter{Filtered quiver varieties}\label{chapter:filtered-quiver-varieties}


DO NOT INCLUDE. REMOVE. DUPLICATE. 
DO NOT INCLUDE. REMOVE. DUPLICATE. 
DO NOT INCLUDE. REMOVE. DUPLICATE. 
DO NOT INCLUDE. REMOVE. DUPLICATE.  
DO NOT INCLUDE. REMOVE. DUPLICATE. 



HAS MORE FILTERED QUIVER VARIETY CONSTRUCTIONS. 


\section{Construction of filtered quiver varieties}
 


Parabolic group actions arise naturally in mathematics. For example, let $B$ be the standard Borel in $GL_n(\mathbb{C})$ and let $\mathfrak{b}=\lie(B)$ be the set of upper triangular matrices in $\mathfrak{gl}_n$, where $\mathfrak{gl}_n$ is the set of all $n\times n$ matrices. 
We may be interested in studying the orbit structure of $B$ acting on $\mathfrak{b}$ by conjugation or we may be interested in studying a variety that has a certain notion of filtrations associated to it. 
Recall from Section~\ref{subsection:GS-resolution-intro} that 
$\mathfrak{b}/B\cong \widetilde{\mathfrak{g}}/G$ so the $B$-orbits on $\mathfrak{b}$ are of significant interest in and of itself. 



Let us now discuss the $B$-adjoint action on $\mathfrak{b}$ further.  
Let $F^{\bullet}:\{ 0\}\subseteq \mathbb{C}^1\subseteq \mathbb{C}^2 \subseteq \ldots \subseteq \mathbb{C}^n$ be the complete standard filtration of vector spaces in $\mathbb{C}^n$.  
Then $\mathfrak{b}$ can be identified with the subspace of linear maps $\mathbb{C}^n\stackrel{f}{\rightarrow} \mathbb{C}^n$ such that $f|_{\mathbb{C}^k}:\mathbb{C}^k\rightarrow \mathbb{C}^k$ for all $k$. 
Since one must preserve the filtration of vector spaces while changing the basis, we have the $B$-action on the domain and the codomain.   
So points of $\mathfrak{b}/B$ correspond to equivalence classes of linear maps preserving the complete standard filtration of vector spaces, where two maps $f$ and $g$ are equivalent if there exists a change-of-basis that will take $f$ to $g$. 



We now give the construction of filtered quiver varieties in the general setting. 
Let $Q=(Q_0,Q_1)$ be a quiver and let $\beta=(\beta_1,\ldots, \beta_{Q_0})\in \mathbb{Z}_{\geq 0}^{Q_0}$ be a dimension vector.  
Let 
$F^{\bullet}:0\subseteq \mathbb{C}^{\gamma_1}\subseteq \mathbb{C}^{\gamma_2}\subseteq \ldots \subseteq \mathbb{C}^{\beta}$ 
be a filtration of vector spaces such that we have the filtration 
$F_i^{\bullet}:0\subseteq \mathbb{C}^{\gamma_1^i}\subseteq \mathbb{C}^{\gamma_2^i}\subseteq \ldots \subseteq \mathbb{C}^{\beta_i}$ of vector spaces at vertex $i$. 
Let $Rep(Q,\beta)$ be the quiver variety in the classical sense (without the filtration of vector spaces imposed). 
Then $F^{\bullet}Rep(Q,\beta)$ is a subspace of $Rep(Q,\beta)$ whose linear maps preserve the filtration of vector spaces at every level.  
Let $P_i\subseteq GL_{\beta_i}(\mathbb{C})$ be the maximal parabolic group preserving the filtration of vector spaces at vertex $i$. 
Then the product $\mathbb{P}:=\prod_{i\in Q_0}P_i$ of parabolic groups acts on 
$F^{\bullet}Rep(Q,\beta)$ as a change-of-basis. 


Now, given a parabolic Lie algebra $\mathfrak{p}=\lie(P)$, 
a general parabolic matrix 
has indeterminates along its block diagonal and upper triangular portion of the matrix and zero below the diagonal blocks.   
We refer to \cite{MR2772068} for a discussion on quiver Grassmannians and quiver flag varieties, which are related to filtered quiver varieties but they are not the same. In the next three sections, we will discuss quiver Grassmannians, quiver flag varieties, and filtered quiver varieties. 
 
\subsection{Quiver Grassmannians}\label{subsection:quiver-grassmannians}
  
Let $\gamma=(\gamma_1,\ldots, \gamma_{Q_0})\in \mathbb{Z}_{\geq 0}^{Q_0}$ be a dimension vector. 
If each $\gamma_k \leq \beta_k$ for each $k\in Q_0$, then we define 
$Gr_{\gamma}(\beta) := \prod_{k\in Q_0}Gr_{\gamma_k}(\beta_k)$ to be the product of Grassmannians,  
where each $Gr_{\gamma_k}(\beta_k)$ parameterizes $\gamma_k$-dimensional subspaces in a $\beta_k$-dimensional vector space. So $Gr_{\gamma}(\beta)$ has dimension $\sum_{k\in Q_0} \gamma_k(\beta_k-\gamma_k)$, which one can obtain by counting the number of indeterminates after row reducing a certain product of matrices, i.e., each matrix corresponding to $Gr_{\gamma_k}(\beta_k)$ is of size $\gamma_k\times \beta_k$ with the rows spanning the $\gamma_k$-dimensional subspace. 
Writing $G_{\beta} :=\prod_{k\in Q_0}GL_{\beta_{k}}(\mathbb{C})$, $Gr_{\gamma}(\beta)$ can also be thought of as $G_{\beta}/P_{\gamma}$, where $P_{\gamma}\subseteq G_{\beta}$ is a product of maximal parabolic matrices with each $P_{\gamma_k}$ stabilizing a $\gamma_k$-dimensional subspace in a $\beta_k$-dimensional vector space. 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
We now define 
\[ \begin{aligned}
 	Gr_{\gamma}^Q(\beta) := 
		\{ ((U(k))_{k\in Q_0}, (W(a))_{a\in Q_1} ) : 
				U(k)\cong \mathbb{C}^{\gamma_k}& \mbox{ is a subspace of } W(k)\cong \mathbb{C}^{\beta_k} \mbox{ and } \\
		   	&W(a)U(i)\subseteq U(j), \mbox{ where } a:i\rightarrow j 
		\}  																																								\\
		\end{aligned}
 \]  to be the universal quiver Grassmannian of $\gamma$-dimensional subrepresentations in $\beta$-dimensional representations of $Q$. 
Note that $Gr_{\gamma}^Q(\beta)$ is a subvariety of the pair $Gr_{\gamma}(\beta)\times Rep(Q,\beta)$, with 
 the product $G_{\beta}$ of invertible matrices acting on $Gr_{\gamma}^Q(\beta)$ diagonally on each factor, i.e., for $(g_k)_{k\in Q_0}\in G_{\beta}$ and having chosen a basis for a sequence $(W(k))_{k\in Q_0}$  of vector spaces (and thus for $(U(k))_{k\in Q_0}$ as well), the $G_{\beta}$-action is given as 
 \[ 
 (g_{k})_{k\in Q_0}. ( ( u_k )_{k\in Q_0}, (W(a))_{a\in Q_1} ) 
 = ((g_k u_k )_{k\in Q_0}, (g_{ha}W(a)  g_{ta}^{-1} )_{a\in Q_1} ),    
 \] where $u_k$ is a vector in $U(k)$ and $W(a)$ is a matrix in  
 $M_{\beta(ha)\times \beta(ta)}$. 
For the mere sake of notational simplicity (this will be apparent in Section~\ref{subsection:quiver-flag-variety} when we discuss quiver flag varieties), 
we may also write  
\[ 
Gr_{\gamma}^Q(\beta) = \{ (U,W) \in Gr_{\gamma}(\beta)\times Rep(Q,\beta): U \mbox{ is a subrepresentation of }W \}.  
\]  


Now consider the projections $Gr_{\gamma}^Q(\beta)\stackrel{p_1}{\longrightarrow} Gr_{\gamma}(\beta)$ and 
$Gr_{\gamma}^Q(\beta)\stackrel{p_2}{\longrightarrow} Rep(Q,\beta)$ onto the two factors, where $p_1$ and $p_2$ are $G_{\beta}$-equivariant maps.  
We will give explicit description of the fibers $p_1^{-1}(U)$ and $p_2^{-1}(W)$. 
For a fixed sequence $(U(k) )_{k\in Q_0}$ of subspaces in the product $Gr_{\gamma}(\beta)$ of Grassmannians,  
we can choose a sequence $( U(k)^{\perp} )_{k\in Q_0}$ of complementary subspaces such that $U(k) \oplus U(k)^{\perp}=W(k)\cong \mathbb{C}^{\beta_k}$ for each vertex $k\in Q_0$. 
Since the preimage of $(U(k))_{k\in Q_0}$ under the first projection map $p_1$ must satisfy $W(a)U(i)\subseteq U(j)$ for each $a:i\rightarrow j$, 
we have 
\[ 
		p_1^{-1}( U ) = 
		  U \times \left( \left[ 
		\begin{array}{cc}
		\Hom_Q(U(i), U(j)) & \Hom_Q(U(i)^{\perp},U(j)) \\
		0 & \Hom_Q(U(i)^{\perp},U(j)^{\perp})   \\
		\end{array}
		\right] \right)_{a:i\rightarrow j}.   
\] 
Thus the fiber of $p_1$ is a vector space of rank 
  \[ \sum_{a:i\rightarrow j, a\in Q_1} \beta_i\gamma_j + (\beta_i-\gamma_i)(\beta_j-\gamma_j)
  =\sum_{a:i\rightarrow j, a\in Q_1} \beta_i \beta_j +\gamma_i\gamma_j - \beta_j\gamma_i,  
  \]  
since $\Hom_Q( U(i),U(j) )$ is a vector space of dimension $\gamma_i\gamma_j$,  
$\Hom_Q( U(i)^{\perp},U(j))$ is a vector space of dimension $(\beta_i-\gamma_i)\gamma_j$, and 
$\Hom_Q( U(i)^{\perp},U(j)^{\perp})$ is a vector space of dimension $(\beta_i-\gamma_i)(\beta_j-\gamma_j)$. 
So $p_1$ is flat. 

  
For $W\in Rep(Q,\beta)$, the preimage $p_2^{-1}(W)$ parameterizes all sequences $(U(k))_{k\in Q_0}$ of subspaces  
  of dimension vector $\gamma$ such that $W(a)U(i)\subseteq U(j)$, 
  where $a:i\rightarrow j$ is an arrow in $Q$. Thus, we identify the fiber of 
    $p_2$ over a fixed representation $W$ as the quiver Grassmannian 
    $Gr_{\gamma}(W) :=p_2^{-1}(W)$ of $W$ of dimension vector $\gamma$; it essentially parameterizes all $\gamma$-dimensional subrepresentations of $W$.  Thus, $p_2$ is projective. 
   Next, we give some examples. 


\begin{example}\label{example:quiver-grassmannian-A1}
Consider the $A_1$-Dynkin quiver (this is the quiver with one vertex and no arrows). 
Let the dimension vector $\beta$ equal $n$. 
Then $Rep(Q,\beta)\cong \mathbb{C}^n$ is an $n$-dimensional vector space. 
Now let the dimension vector $\gamma$ be $m \leq n$. 
We obtain $Gr_{m}^{Q}(n) =Gr_m(n)\times \mathbb{C}^n$ 
with the quiver Grassmannian $Gr_m(\mathbb{C}^n) = Gr_m(n)$ coinciding with the classical notion of a Grassmannian.  
\end{example} 


\begin{example}\label{example:quiver-grassmannian-A2}
Consider the $A_2$-Dynkin quiver 
$\xymatrix@-1pc{ \stackrel{1}{\bullet} \ar[rr]^a & & \stackrel{2}{\bullet}}$ and let $\beta =(n_1,n_2)$. Let $\gamma = (m_1, m_2)$ with $m_{k}\leq n_k$ for $k=1,2$. Then 
for $W\in M_{n_2\times n_1}=Rep(Q,\beta)$,  
the quiver Grassmannian $Gr_{(m_1,m_2)}(W)$ is a closed subvariety of $Gr_{m_1}(\mathbb{C}^{n_1})\times Gr_{m_2}(\mathbb{C}^{n_2})$ which satisfies 
$W(U(1))\subseteq U(2)$, where $\dim (U(i))=m_i$, $i=1,2$.    
\end{example}





\subsection{Quiver flag varieties}\label{subsection:quiver-flag-variety}

In this section, we generalize Section~\ref{subsection:quiver-grassmannians}   
by discussing the notion of quiver flag varieties. 
These varieties also appear in the literature as quiver flag manifolds. 
Similar as before, fix a dimension vector $\beta=(\beta_1,\ldots, \beta_{Q_0})$. Let $\gamma^{(1)}, \ldots, \gamma^{(l)}\in \mathbb{Z}_{\geq 0}^{Q_0}$
be dimension vectors with coordinates 
$\gamma^{(k)}=(\gamma_1^{(k)},\ldots, \gamma_{Q_0}^{(k)})$ 
satisfying $\sum_{k=1}^l \gamma_i^{(k)}\leq \beta_i$ for each $i\in Q_0$. 
Let $\gamma^{(l+1)}\in \mathbb{Z}_{\geq 0}^{Q_0}$ such that  
$\sum_{k=1}^{l+1} \gamma_i^{(k)} = \beta_i$ for each $i\in Q_0$.  
Define $Fl_{\gamma^{\bullet}}(\beta) := \prod_{i\in Q_0} Fl_{\gamma_i^{\bullet}}(\beta_i)$  
to be the product of flag varieties,  
where each $Fl_{\gamma_i^{\bullet}}(\beta_i)$
is the usual flag variety parametrizing flags of subspaces 
\[ 0 \subseteq U_i^{(1)}\subseteq U_i^{(2)} \subseteq \ldots \subseteq U_i^{(l)} \subseteq W(i)
\] 
   with $\dim U_i^{(k)} = \sum_{u=1}^k \gamma_i^{(u)}$. 
We define the universal quiver flag to be 
\begin{equation}\label{equation:universal-quiver-flag}
  \begin{aligned}
  Fl_{\gamma^{\bullet}}^Q(\beta) := 
  \{ &(U^{(1)},\ldots, U^{(l)}, W) \in Fl_{\gamma^{\bullet}}(\beta)\times Rep(Q,\beta): 
    0 \subseteq U^{(1)} \subseteq U^{(2)} \subseteq \ldots \subseteq U^{(l)} \subseteq W \mbox{ is } \\
    &\mbox{ a chain of subrepresentations of }W   
    \mbox{ and } W(a)U_i^{(k)}\subseteq U_j^{(k)}\:\: \forall \: a:i\rightarrow j \mbox{ and }  
    \forall \: 1\leq k\leq l
            \}.   \\ 
    \end{aligned}
 \end{equation}

Consider the two $G_{\beta}$-equivariant projections $Fl_{\gamma^{\bullet}}^Q(\beta)\stackrel{p_1}{\longrightarrow} Fl_{\gamma^{\bullet}}(\beta)$
and 
$Fl_{\gamma^{\bullet}}^Q(\beta)\stackrel{p_2}{\longrightarrow} Rep(Q,\beta)$. 
First, let us view $U_i^{(k)}$ as subspaces in $W(i)$ for each $i\in Q_0$. 
The fiber of $p_1$ over the tuple 
$(U^{(1)},\ldots, U^{(l)})$ is 
again a homogeneous vector bundle isomorphic to 
\begin{equation}\label{eq:quiver-flag-vector-bundle} 
\bigoplus_{a\in Q_1}
\left( 
\bigoplus_{k=1}^{l}\Hom\left(U_{ta}^{(k)}/U_{ta}^{(k-1)}, U_{ha}^{(k)} \right)
\oplus \Hom\left(W(ta)/U_{ta}^{(l)},W(ha)\right)
\right) 
\end{equation}
where $U_{ta}^{(k)}/U_{ta}^{(k-1)}:=\{v\in U_{ta}^{(k)}:v\perp u \:\:\forall u\in U_{ta}^{(k-1)} \}$, 
$W(ta)/U_{ta}^{(l)} := \{ v\in W(ta): v\perp u \:\:\forall u\in U_{ta}^{(l)} \}$, 
and $U_{ta}^{(0)}:=0$. So $p_1$ is flat. 
On the other hand, 
$p_2^{-1}(W)$ parameterizes all flags 
$0 \subseteq U^{(1)} \subseteq U^{(2)} \subseteq \ldots \subseteq U^{(l)} \subseteq W$ of subspaces with prescribed dimension vectors $\gamma^{(k)}$ with each $U^{(k)}$ being a subrepresentation of $U^{(k+1)}$ and $U^{(l)}$ being a subrepresentation of $W$. So $p_2$ is projective.  
The fiber $p_2^{-1}(W)=Fl_{\gamma^{\bullet}}(W)$ of $p_2$ over $W$ is called the quiver flag variety. 


\begin{example}\label{example:quiver-flag-A1}
Consider the $A_1$-quiver and let $\beta=n$. 
Let $l=n-1$ and let $\gamma^{(i)}=i$ for $1\leq i\leq l$.  
Then the quiver flag variety $Fl_{\gamma^{\bullet}}(\mathbb{C}^n)$ 
is isomorphic to the complete flag variety in $\mathbb{C}^n$. 
\end{example}  
 
\begin{example}\label{example:quiver-flag-generalizing-grassmannian}
Let $Q$ be any quiver and let $l=1$ to obtain the quiver Grassmannian from Section~\ref{subsection:quiver-grassmannians}. 
\end{example} 



It is worth mentioning that when rewriting the direct sum of vector bundles in (\ref{eq:quiver-flag-vector-bundle}) as a product of matrices (one matrix for each arrow $a\in Q_1$), each matrix has the form of a parabolic matrix. The next section investigates the fibers of $p_1$. 



\subsection{Filtered quiver varieties}\label{subsection:filtered-quiver-varieties}


Filtered quiver varieties are precisely the fibers of $p_1$ over filtered vector spaces in Section~\ref{subsection:quiver-flag-variety}. 
A more direct construction is given as follows: 
let $Q$ be any quiver. 
Fix a set of dimension vectors $\gamma^{(1)},\ldots, \gamma^{(l)}, \beta \in \mathbb{Z}_{\geq 0}^{Q_0}$ such that $\sum_{k=1}^{l} \gamma_{i}^{(k)} \leq \beta_{i}$ for each $i\in Q_0$. 
Let $F^{\bullet}: 0 \subseteq U^{(1)} \subseteq U^{(2)} \subseteq \ldots \subseteq U^{(l)} \subseteq W$ be a flag of subspaces such that 
$\dim U_i^{(k)} = \sum_{u=1}^k \gamma_i^{(u)}$ for each $i\in Q_0$. 
 

  
%We make a note that filtered quivers with \textit{any} prescribed filtration of dimension vectors 
%may not exist or such notion may be ambiguous, i.e., the filtration of dimension vectors depends on the quiver $Q$ (see Example~\ref{example:A3-quiver-prelim}), which is our reason for giving Definition~\ref{definition:admissible-dimension-vectors}.  
 


  
 
\begin{definition}\label{definition:filtered-quiver-representation}   
The filtered quiver variety is  
\[ 
F^{\bullet}Rep(Q,\beta):= \{ W\in Rep(Q,\beta):
W(U_{ta}^{(k)})\subseteq U_{ha}^{(k)}\:\: \forall \: 1\leq k\leq l, \:\:\forall \:a\in Q_1
\}. 
\] 
If $P_i\subseteq GL_{\beta_i}(\mathbb{C})$ is a parabolic subgroup acting as a change-of-basis while preserving the filtration of vector spaces at vertex $i\in Q_0$, 
then $P_{\beta}:= \prod_{i\in Q_0}P_i$ naturally acts on $F^{\bullet}Rep(Q,\beta)$.   
\end{definition}  

A filtered quiver variety is a representation space where the filtration is a structure on a representation, not on the quiver itself. 
We will write $\mathbb{P}:= P_{\beta}$, where all information on the filtration of vector spaces is suppressed throughout this thesis. 



  

\begin{remark}\label{remark:filtration-on-framed-quiver}    
We will construct a 
\textbf{framed filtered quiver variety}, 
denoted as 
$F^{\bullet}Rep({Q}^{\dagger},\beta^{\dagger} )$, as follows: 
the filtration $F^{\bullet}$ on the framed variety 
$F^{\bullet}Rep({Q}^{\dagger},\beta^{\dagger} )$ 
modifies vector spaces assigned to vertices in $Q_0$,   
but not those vector spaces assigned to framed vertices 
$Q_0^{\natural}$.  
Writing the dimension vector for a framed quiver as 
$\beta^{\dagger}=(\beta,\beta^{\natural})$, 
$P_{\beta}\times \Inoindex_{\beta^{\natural}}\hookrightarrow P_{\beta}\times P_{\beta^{\natural}}=: P_{\beta^{\dagger}}$  
naturally acts on  
$F^{\bullet}Rep({Q}^{\dagger},\beta^{\dagger})$, where $\Inoindex_{\beta^{\natural}}=\prod_{i\in Q_0^{\natural}} \Inoindex_{\beta_i^{\natural}}$ 
is a product of identity matrices, one for each framed vertex; 
we will refrain from writing $\Inoindex_{\beta^{\natural}}$ 
and simply write $P_{\beta}$. 
If the tail of the underlying arrow (or more generally, path) 
of a general representation is not a framed vertex, then the general representation must preserve the fixed filtration $F^{\bullet}$ of vector spaces at both the head and the tail of the underlying arrow (or path); 
such representation is possibly block upper triangular and has indeterminates in those entries that are not zero. 
However, all other linear maps whose tail is a framed vertex, i.e., 
these are of the form 
$W(\iota_i)\in\Hom(\mathbb{C}^{\beta_i^{\natural}}, \mathbb{C}^{\beta_i} )$,  
have indeterminates in all entries 
(since we do not impose a fixed filtration of vector spaces on framed vertices).  
\end{remark}  
    
  
 
  
     


\begin{remark}\label{remark:filtration-on-a-bipartite-graph} 
Using notations in Construction~\ref{construction:bipartite-quiver},  
we construct a 
\textbf{filtered bipartite quiver variety} 
as follows:    
the filtration $F_i^{\bullet}$ 
of vector spaces that is imposed on the vector space $W(i)$ at vertex $i \in Q_0$ 
is also imposed on $W(i')$, where $i' \in Q_0'$,  
such that representations of arrows in $Q_1'$ 
preserve the filtration.  
Viewing $W(c_i)$  
as a general representation which preserves the filtration of vector spaces at both $i$ and $i'$, 
one may identify $W(c_i)$ with 
$\mathfrak{p}_{\beta_i}\subseteq \mathfrak{gl}_{\beta_i}$ 
(thus $W(c_i)$ is a block diagonal upper triangular square matrix)  
and one may view $W(a')$ as   
$\mathfrak{p}_{\beta_{ha'}}\subseteq \mathfrak{gl}_{\beta_{ha'}}$ 
if and only if the filtration of vector spaces at the tail of $a$ 
equals the filtration of vector spaces at the head of $a$. 
We will denote the filtered bipartite quiver variety as  
$F^{\bullet}Rep(\widehat{Q},\widehat{\beta})$. 
The product $P_{\widehat{\beta}}:=P_{\beta}\times P_{\beta'}$ 
of parabolic groups acts on the filtered bipartite representation space by acting as a change-of-basis on representations of arrows in $\widehat{Q}$. 
\end{remark}  
  
   
   
   
 
\begin{remark}\label{remark:filtered-opposite-quiver-variety} 
Let $Q^{op}$ be the opposite quiver as defined in 
Definition~\ref{definition:opposite-quiver} and let 
$\beta\in \mathbb{Z}_{\geq 0}^{Q_0}$ 
be the dimension vector. 
Let $F^{\bullet}$ be a fixed filtration of vector spaces over vertices of $Q$. 
We will define \textbf{filtered opposite quiver variety} 
$F^{\bullet}Rep(Q^{op},\beta)$ to be the representation space whose general representation 
$W(a^{op})$ 
of arrows 
$a^{op}\in Q_1^{op}$  
preserves the filtration of vector spaces over each vertex, where the product 
$P_{\beta}$ of parabolic groups acts on the representation space as a change-of-basis. 
Note that $W(a^{op})$ has an upper triangular form. 
\end{remark} 
  
   
   
   
   
   
   
   
   
   
  
 
\begin{remark}\label{remark:double-quiver-filtered-setting}
Using Notation~\ref{construction:double-quiver-classical-setting}, we will define the filtered representation space of a double quiver as 
$F^{\bullet}Rep(\overline{Q},\overline{\beta}) := F^{\bullet}Rep(Q,\beta)\times F^{\bullet}Rep(Q^{op},\beta)$, where $Q^{op}=(Q_0,Q_1^{op})$.  
The group $P_{\overline{\beta}}=P_{\beta}$ acts on $F^{\bullet}Rep(\overline{Q},\overline{\beta})$ by acting on  
$F^{\bullet}Rep(Q,\beta)$ and $F^{\bullet}Rep(Q^{op},\beta)$ as a change-of-basis. 
\end{remark}   
 
 
Note that filtered quiver varieties for double quivers are not the same as the cotangent bundle of filtered quiver varieties because 
$W(a^{op})$ in $F^{\bullet}Rep(Q^{op},\beta)$ still has block upper triangular form. 
Remark~\ref{remark:cotangent-bundle-of-filtered-reps} 
describes a notion of the cotangent bundle of filtered quiver varieties.  

 
\begin{remark}\label{remark:cotangent-bundle-of-filtered-reps}   
Let 
 \[ 
 \begin{aligned} 
 &F_i^{\bullet}: \{0\} = W_i^{(0)} \subseteq W_i^{(1)} \subseteq \ldots \subseteq W_i^{(l)} \cong \mathbb{C}^{\beta_i},  \\ 
 &G_i^{\bullet}: \mathbb{C}^{\beta_i} = (W_i^{(0)})^{\perp} \supseteq (W_i^{(1)})^{\perp} \supseteq \ldots \supseteq (W_i^{(l)})^{\perp} \cong (\mathbb{C}^{\beta_i})^{\perp} = \{0\} 
   %V^{(0)} \subseteq V^{(1)} \subseteq \ldots \subseteq V^{(l)} \cong \mathbb{C}^{\alpha}, \\ 
\end{aligned}
\]   
		be two filtrations of vector spaces, where $i\in Q_0$ and  
		$(W_i^{(k)})^{\perp}$ is the quotient space $\mathbb{C}^{\beta_i}/W_i^{(k)}$; that is, $(W_i^{(k)})^{\perp}$ 
		could be thought of as the subspace of $\mathbb{C}^{\beta_i}$   
whose first $k$ coordinates are zero.   
We define $F^{\bullet}Rep(Q,\beta)^*$   
to be $G^{\bullet}Rep(Q^{op},\beta)$ that preserves $G^{\bullet}$. 
% 
Then 
\[ F^{\bullet}Rep(Q,\beta) \times F^{\bullet}Rep(Q,\beta)^* \longrightarrow \mathbb{C}, 
\hspace{4mm}
					(W,W^*)\mapsto \Tr(WW^*)
\]   
is a perfect pairing.  
%  \[ 
%  	\Hom(	(\mathbb{C}^{\beta})^{F^{\bullet}},
%	   		(\mathbb{C}^{\alpha})^{G^{\bullet}}	 )  
%	   		\times 
%		\Hom(	(\mathbb{C}^{\beta})^{F^{\bullet}},
%	   		(\mathbb{C}^{\alpha})^{G^{\bullet}}	 )^* \longrightarrow \mathbb{C}
%   \] given by $(A,B)\mapsto \Tr(AB^t)=\Tr(B^t A)$. 
%   
%   
%    
%
The cotangent bundle $T^*F^{\bullet}Rep( Q,\beta)$ of a filtered representation space is defined to be 
$F^{\bullet}Rep(Q,\beta)\times F^{\bullet}Rep(Q,\beta)^*$. 
Since the action of $P_{\beta}$ on $F^{\bullet}Rep( Q,\beta)$ is induced onto 
the cotangent bundle, we will write $P_{\beta^*} :=P_{\beta}$, where $\beta^*$ is the dimension vector associated to $T^*F^{\bullet}Rep( Q,\beta)$.   
\end{remark}
  
%In Remark~\ref{remark:cotangent-bundle-of-filtered-reps}, transposed matrices are the reps associated to opposite arrows.   
   
 
 
\begin{example}\label{example:quiver-with-oriented-path}  
Consider the $2$-Kronecker quiver with filtered representation:  
\[ 
\xymatrix@R-1pc{ 
\mathbb{C}^5 	\ar@{-}[d]   					&& \mathbb{C}^4 \ar@{-}[d]  \\
\mathbb{C}^4 	\ar@{-}[d]   					&& \mathbb{C}^3 \ar@{-}[d]  \\
\mathbb{C}^3 	\ar@{-}[d] 						&& \mathbb{C}^1 \ar@{-}[d]  \\
\mathbb{C}^0 						 						&& \mathbb{C}^0 						 \\ 
\stackrel{W(1)}{\bullet} \ar@/^/[rr]| {W(a_1)} 	&& \stackrel{W(2).}{\bullet} \ar@/^/[ll]|{W(a_2)}
} 
\]
Then 
\[ W(a_1) = \left[ \begin{array}{ccccc} 
*&*&*& *&* \\ 
0&0&0& *&* \\
0&0&0& *&* \\
0&0&0& 0&* \\
\end{array} 
\right] \mbox{ while }
W(a_2) = \left[ \begin{array}{cccc} 
*&*&*&* \\ 
*&*&*&* \\ 
*&*&*&* \\ 
0&*&*&* \\ 
0&0&0&* \\ 
\end{array}
\right].  
\]   
Note that both $W(a_1)$ and $W(a_2)$ have block upper triangular form. 
\end{example} 




    
   
   
 
\begin{remark}\label{remark:filtration-framed-bipartite-quiver} 
We will construct 
\textbf{framed filtered bipartite quiver variety} 
$F^{\bullet}Rep(\widehat{Q}^{\dagger},\widehat{\beta}^{\dagger})$. 
This construction combines 
Remark~\ref{remark:filtration-on-a-bipartite-graph} 
and 
Remark~\ref{remark:filtration-on-framed-quiver}, 
where the filtration of vector spaces is only imposed on vector spaces assigned to vertices 
$Q_0$ and to $Q_0'$, 
i.e.,
the filtration is not imposed on the framed vertices 
$Q_0^{\natural}$ and $(Q_0^{\natural})'$.   
Thus, 
all linear maps 
(except those whose domain or codomain correspond to the vector space at a framed vertex) 
preserve the filtration; 
a general representation of these linear maps has indeterminates in block upper triangular form while a general representation whose tail or head of the underlying quiver is a framed vertex has indeterminates in all entries. 
More precisely, 
representations in 
$F^{\bullet}Rep(\widehat{Q}^{\dagger},\widehat{\beta}^{\dagger})$ 
are defined in a compatible way as follows: 
$W(a')$ is the set of all maps which preserves filtrations of vector spaces if both the head and the tail of $a'$ are not framed vertices, 
$W(\iota_i')$ is the set of all linear maps from the vector space at a framed vertex $i^{\natural}$ 
to the vector space at a nonframed vertex $i'\in Q_0'$ 
(thus, the general representation $W(\iota_i')$ is 
$\Hom(\mathbb{C}^{\beta_i^{\natural}},\mathbb{C}^{\beta_{i'}} )$), 
$W(c_i)$ 
is a map preserving the fixed filtration of vector spaces from 
$W(i)$ to $W(i')$, 
where $i\in Q_0$ 
(so a general representation $W(c_i)$ 
is $\mathfrak{p}_{\beta_i}$), 
and finally, $W(c_{i^{\natural}})$ is the identity matrix from the vector space $W(i^{\natural})$ to the vector space $W((i^{\natural})')$, where both $i^{\natural}$ and $(i^{\natural})'$ are framed vertices.  
The vector space 
$F^{\bullet}Rep(\widehat{Q}^{\dagger},\widehat{\beta}^{\dagger})$ 
is naturally acted upon by $P_{\widehat{\beta}} = P_{\beta}\times P_{\beta'}$. 
\end{remark} 





First, we will give the notion of doubling a filtered quiver variety. 
Unlike the classical setting, the notion of doubling is not the same as the cotangent bundle of a filtered quiver variety. 
\begin{remark}\label{remark:doubling-a-filtered-quiver-variety}
Let $Q=(Q_0,Q_1)$ be a quiver and let $\beta\in \mathbb{Z}_{\geq 0}^{Q_0}$ be a dimension vector. 
Let $F^{\bullet}$ be fixed filtrations of vector spaces over vertices of $Q$. 
Let $F^{\bullet}Rep(Q,\beta)$ 
be a filtered representation space of 
$Q$ with dimension vector $\beta$ such that representations $W(a)$ of arrows $a\in Q_1$ 
preserve the filtration of vector spaces assigned to the tail 
$ta$ of $a$ and to the head $ha$ of $a$. 
Define $\overline{Q}=(\overline{Q}_0,\overline{Q}_1)$ to be the double quiver as defined in Construction~\ref{construction:double-quiver-classical-setting}. 
We will define 
\textbf{filtered double quiver variety}  
$F^{\bullet}Rep(\overline{Q},\overline{\beta}) =
F^{\bullet}Rep(Q,\beta)\times F^{\bullet}Rep(Q^{op},\beta)$ 
to be the following: for each arrow $a\in Q_1$,  
%with $W(a)\in F^{\bullet}Rep(Q,\beta)$, 
$W(a^{op})\in F^{\bullet}Rep(Q^{op},\beta)$ is the linear map $W(a^{op}):W(ha)\rightarrow W(ta)$ 
preserving the filtration of vector spaces at $W(ha)$ 
and at $W(ta)$.  
Note that $W(a^{op})$ also has an upper triangular form. 
\end{remark}




\begin{remark}\label{remark:double-framed-filtered-quiver-variety} 
Let $Q$ be a quiver and let $\beta\in \mathbb{Z}_{\geq 0}^{Q_0}$ be a dimension vector. 
Let $F^{\bullet}$ be a fixed filtration of vector spaces over vertices of $Q$. 
Consider the double framed quiver $\overline{Q}^{\dagger}$ in Construction~\ref{construction:double-framed-quiver}. 
We define 
\textbf{double framed filtered quiver variety} 
as 
$F^{\bullet}Rep(\overline{Q}^{\dagger},\overline{\beta}^{\dagger})
= F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})\times 
F^{\bullet}Rep((Q^{\dagger})^{op},\beta^{\dagger})$, where 
$(Q^{\dagger})^{op}=(Q_0,(Q_1^{\dagger})^{op})$.  
Here, 
the product $P_{\beta}$ of parabolic groups acts on 
$F^{\bullet}Rep(\overline{Q}^{\dagger},\overline{\beta}^{\dagger})$ 
as a change-of-basis on vector spaces over nonframed vertices while preserving the filtration of vector spaces.  
\end{remark}  

 


Before we define the cotangent bundle of a filtered quiver variety,   
let $\mathfrak{b}\subseteq \mathfrak{gl}_n$   
be the set of upper triangular matrices. 
We want to understand $\mathfrak{b}^*$. 
So consider 
\[ \mathfrak{gl}_n \stackrel{\Psi}{\longrightarrow}\mathfrak{b}^* =\Hom(\mathfrak{b}, \mathbb{C}), 
\hspace{4mm} \mbox{ where }
- \mapsto (s\mapsto \Tr(- s)). 
\]   
For $r\in \mathfrak{n}^+$, which is the set of strictly upper triangular matrices, $\Tr(rs)=0$. 
So $\Psi$ factors through  
$\mathfrak{gl}_n/\mathfrak{n}^+$. 
Since $\ker\Psi=\mathfrak{n}^+$, 
we have  
$\mathfrak{gl}_n/\mathfrak{n}^+ \cong \mathfrak{b}^*$.  





In slight more generality, let $\mathfrak{p}\subseteq \mathfrak{gl}_n$ be a block upper triangular parabolic Lie algebra. We want to understand $T^*\mathfrak{p}=\mathfrak{p}\times \mathfrak{p}^*$ in terms of filtered quiver varieties.  
So consider 
\[ \mathfrak{gl}_n\longrightarrow \mathfrak{p}^*=\Hom(\mathfrak{p},\mathbb{C}),
\hspace{4mm} 
- \mapsto (s\mapsto \Tr(- s)). 
\] 
Let $r\in \nil(\mathfrak{p})$, where $\nil(\mathfrak{p})$ is the nilradical of $\mathfrak{p}$, i.e., 
\[ \xymatrix{0 \ar[rr] & & \nil(\mathfrak{p}) \ar[rr] & & \mathfrak{p} \ar[rr] & &  \mathfrak{l} \ar[rr] & & 0
}
\] is a short exact sequence such that $\mathfrak{p}/\nil(\mathfrak{p})\cong \mathfrak{l}$, where $\mathfrak{l}$ is the Levi subalgebra of $\mathfrak{p}$. 
For $r\in \nil(\mathfrak{p})$, which is a maximal nilpotent ideal of $\mathfrak{p}$, $\Tr(rs)=0$. Thus, $\mathfrak{gl}_n/\nil(\mathfrak{p})\cong \mathfrak{p}^*$. 

 

   
\begin{remark}\label{remark:cotangent-bundle-of-filtered-quiver-variety}  
We will now give a canonical construction of the 
\textbf{cotangent bundle of a filtered quiver variety}.  
Let 
$F^{\bullet}Rep(Q,\beta)$ 
be a filtered quiver variety, where the filtration $F^{\bullet}$ of vector spaces is 
\[ 
F_i^{\bullet}: 0 \subseteq \mathbb{C}^{\gamma_1}\subseteq \mathbb{C}^{\gamma_2}\subseteq \ldots \subseteq \mathbb{C}^{\gamma_{l-1}} \subseteq \mathbb{C}^{\beta_i} 
\] 
at each vertex $i$ such that the filtration (except the top dimensional vector space) is the same at each vertex. Furthermore, we will restrict to those filtrations and dimension vectors such that if the filtration $F_i^{\bullet}$ at vertex $i$ (with the top dimensional vector space omitted) is not the same as the filtration $F_j^{\bullet}$ at vertex $j$ (with the top dimensional vector space omitted) where $i\not=j$, then $\beta_i=0$ or $\beta_j=0$.  
We will define 
$T^*F^{\bullet}Rep(Q,\beta)=F^{\bullet}Rep(Q,\beta)\times F^{\bullet}Rep(Q,\beta)^*$, where 
\[ F^{\bullet}Rep(Q,\beta)^* = Rep(Q^{op},\beta)/\nil(F^{\bullet}Rep(Q^{op},\beta)). 
\]   
Let $Q^{\dagger}$ be the framed quiver as given in Construction~\ref{construction:framing-to-construct-semi-invariants} and Remark~\ref{remark:filtration-on-framed-quiver}.  
We will define the 
\textbf{cotangent bundle of framed filtered quiver variety} 
as the following: 
\[ T^*F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})
= F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})
\times 
F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})^*, 
\] 
where 
\[
\begin{aligned} 
F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})^*
&= Rep(Q^{op},\beta)/\nil(F^{\bullet}Rep(Q^{op},\beta)) 
\times 
\Hom(\mathbb{C}^{\beta^{\natural}},\mathbb{C}^{\beta})^* \\ 
&\cong  
Rep(Q^{op},\beta)/\nil(F^{\bullet}Rep(Q^{op},\beta)) 
\times 
\Hom(\mathbb{C}^{\beta}, \mathbb{C}^{\beta^{\natural}}),  \\ 
\end{aligned} 
\] 
with $\Hom(\mathbb{C}^{\beta}, \mathbb{C}^{\beta^{\natural}}) = \prod_{i\in Q_0} 
\Hom(\mathbb{C}^{\beta_i}, \mathbb{C}^{\beta_i^{\natural}})$. 
%Note that when 
%$F^{\bullet}$ is the trivial filtration, i.e., $F^{\bullet}:0\subseteq \mathbb{C}^{\beta_i}$ for each vertex $i$, 
%then our construction coincides with the classical setting since a reductive group has no nilradical. 
\end{remark} 



 
We will use the bipartite double framed quiver in Construction~\ref{construction:bipartite-double-framed-quiver} 
to construct bipartite cotangent bundle of framed filtered quiver variety. 
 
 
 
 
\begin{remark}\label{remark:bipartite-cotangent-bundle-double-framed-filtered-quiver}
We will now give the construction of the 
\textbf{bipartite cotangent bundle of framed filtered quiver variety}, 
which is denoted as 
$\bipartite(T^*F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger}))$. 
Let 
$Q$ be any quiver and let $\beta^{\dagger}:=(\beta,\beta^{\natural})\in (\mathbb{Z}_{\geq 0}^{Q_0})^2$ be a dimension vector. 
Since the underlying quiver of $T^*F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})$ equals the underlying quiver of 
$F^{\bullet}Rep(\overline{Q}^{\dagger},\overline{\beta}^{\dagger})$, 
$\bipartite(T^*F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger}))$ 
is a variety whose underlying quiver is the quiver in 
Construction~\ref{construction:bipartite-double-framed-quiver} with representations of arrows given as follows: 
to each nonframed vertex $i\in \widehat{Q}_0$, we impose a filtration $F_i^{\bullet}$ of vector spaces such that the filtration of vector spaces at $i$ equals the filtration of vector spaces at $i'$, and to each framed vertex 
$i^{\natural}\in Q_0^{\natural}$ 
and 
$(i^{\natural})'\in (Q_0^{\natural})'$, 
we simply assign the vector space 
$\mathbb{C}^{\beta_i^{\natural}}$. 
We will write the set of arrows $(\overline{Q}_1^{\dagger})'$ as 
\[ 
(\overline{Q}_1^{\dagger})'= (Q_1^{\dagger}\cup (Q_1^{\dagger})^{op})'
= (Q_1\cup Q_1^{\natural}\cup Q_1^{op}\cup (Q_1^{\natural})^{op})'
= \widehat{Q}_1\cup \widehat{Q_1^{\natural}} 
				\cup \widehat{(Q_1^{op})} \cup \widehat{(Q_1^{\natural})^{op}}.  
\] 
For those $c_{i^{\natural}}\in \widehat{Q_1^{\natural}}$ 
where 
$W(c_i^{\natural}):\mathbb{C}^{\beta_i^{\natural}}\longrightarrow \mathbb{C}^{\beta_i^{\natural}}$, 
we will assign $W(c_i^{\natural}):=\Inoindex_{\beta_i^{\natural}}$. 
To each arrow 
$c_i\in \widehat{Q}_1$, a general representation $W(c_i)$ 
preserves the filtration of vector spaces at vertices $i$ and $i'$. 
This implies that $W(c_i)$ 
has the form of block diagonal upper triangular parabolic group $\mathfrak{p}_{\beta_i}$. 
For those $a'\in \widehat{Q}_1$, 
$W(a')\in F^{\bullet}Rep(\widehat{Q},\widehat{\beta})$, 
i.e., 
representations of $a'$ 
preserve the filtration of vector spaces at both the head and the tail of $a'$. 
For those 
$(a^{op})'\in \widehat{(Q_1^{op})}$, 
a general representation $W( (a^{op})')$ 
is isomorphic to a representation 
in $Rep(\widehat{Q^{op}},\widehat{\beta})/
\nil(F^{\bullet}Rep(\widehat{Q^{op}},\widehat{\beta}))$. 
And finally, for those $\iota_i'\in \widehat{Q_1^{\natural}}$ 
where  
$W(\iota_i'):\mathbb{C}^{\beta_i^{\natural}}\longrightarrow \mathbb{C}^{\beta_{i'}}$, 
the general representation of $W(\iota_i')$ is 
$\Hom(\mathbb{C}^{\beta_i^{\natural}}, \mathbb{C}^{\beta_{i'}})$, 
while for those 
$\gamma_i'\in \widehat{(Q_1^{\natural})^{op}}$ 
where 
$W(\gamma_i'):\mathbb{C}^{\beta_{i'}}\longrightarrow \mathbb{C}^{\beta_i^{\natural}}$
a general representation of $W(\gamma_i')$ is
$\Hom(\mathbb{C}^{\beta_{i'}}, \mathbb{C}^{\beta_i^{\natural}})$. 




We define 
\[ \bipartite(F^{\bullet}Rep(Q,\beta)\times  
Rep(Q^{op},\beta)  
\times  
\Hom(\mathbb{C}^{\beta^{\natural}},\mathbb{C}^{\beta}) 
\times  
\Hom(\mathbb{C}^{\beta},\mathbb{C}^{\beta^{\natural}})) 
\] 
to be the variety whose underlying quiver is the bipartite double framed quiver such that  
\[  
\begin{aligned} 
\ker[  
\bipartite(F^{\bullet}Rep(Q,\beta) 
&\times  
Rep(Q^{op},\beta)  
\times  
\Hom(\mathbb{C}^{\beta^{\natural}},\mathbb{C}^{\beta}) 
\times  
\Hom(\mathbb{C}^{\beta},\mathbb{C}^{\beta^{\natural}})) \\
&\twoheadrightarrow
\bipartite(T^*F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger}))] = \nil(F^{\bullet}Rep(\widehat{Q^{op}},\widehat{\beta})).  \\ 
\end{aligned}  
\]   
\end{remark}   
  
   
 
 




\section{The cotangent bundle of the Grothendieck-Springer resolution}\label{section:cotangent-bundle-of-GS-resolutions} 

We begin with some propositions in symplectic geometry. 

\begin{proposition}\label{proposition:group-action-on-product-space}
Let $G$ be a Lie group with Hamiltonian action on symplectic manifolds 
$(M_1,\omega_1)$ and $(M_2,\omega_2)$ with moment maps 
$\mu_1:M_1\rightarrow \mathfrak{g}^*$ and 
$\mu_2:M_2\rightarrow \mathfrak{g}^*$. 
Then the diagonal action of $G$ on $M_1\times M_2$ is Hamiltonian with $\mu:M_1\times M_2 \rightarrow \mathfrak{g}^*$, 
where $\mu(p_1,p_2)=\mu_1(p_1)+\mu_2(p_2)$ 
for $p_i\in M_i$.  
\end{proposition}



Consider $M=T^*(G\times \mathfrak{b}\times \mathbb{C}^n)$ under the $G\times B$  action. We want to relate $M$ with 
$T^*(G\times_B \mathfrak{b}\times \mathbb{C}^n)=T^*(\widetilde{\mathfrak{g}}\times \mathbb{C}^n)$ under the $B$-action. 
Let $B$ act on $G\times \mathfrak{b}$ via $b.(g,r)=(gb^{-1},brb^{-1})$, 
Chriss and Ginzburg prove the identification 
$G\times_B \mathfrak{b}=\{(x,\mathfrak{b})\in \mathfrak{g}\times G/B:x\in \mathfrak{g} \}$ (\cite{MR2838836}, Corollary 3.1.33). 
Let $(\mathbb{C}^n)^*$ be the dual of $\mathbb{C}^n$. 
That is, if we think of  $i\in \mathbb{C}^n$ as a column vector, then we should think of $j\in (\mathbb{C}^n)^*$ as a row vector. 
Let $G\times B$ act on $T^*(G\times \mathfrak{b}\times \mathbb{C}^n)$ in the following way:  
for $g\in G$ and  
$(g',\theta,r,s,i,j)\in G\times \mathfrak{g}\times\mathfrak{b}\times \mathfrak{b}^*\times \mathbb{C}^n \times (\mathbb{C}^n)^*$, 
\begin{equation}\label{equation:constructing-gs-resolution-g-action}
g.(g',\theta,r,s,i,j) = (g'g^{-1},g\theta g^{-1},r,s,gi,jg^{-1})
\end{equation}
and for $b\in B$ and $(g',\theta,r,s,i,j)$, 
\begin{equation}\label{equation:constructing-gs-resolution-b-action}  
b.(g',\theta,r,s,i,j) = (g'b^{-1},b\theta b^{-1},brb^{-1},bsb^{-1}, i,j). 
\end{equation}

We will explain the identification of 
$\mathfrak{b}^*\cong \mathfrak{gl}_n/\mathfrak{u}$. 
Consider the trace pairing 
$\mathfrak{b}\times \mathfrak{gl}_n \stackrel{\psi}{\longrightarrow}\mathbb{C}$ 
where $(r,s)\mapsto \Tr(rs)$. This map is $B$-equivariant since 
\[ 
\psi(b.(r,s)) =\psi(brb^{-1},bsb^{-1}) =\Tr (brb^{-1}bsb^{-1}) = \Tr(rs)=\psi(r,s)  
\] 
and nondegenerate since 
$\psi(r,s)=\Tr(rs)=0$ for all $s\in \mathfrak{gl}_n$ implies $r=0\in \mathfrak{b}$ by a direct calculation. 
So $\mathfrak{gl}_n$ is a space of linear functionals on $\mathfrak{b}$ via 
$s\mapsto \Tr(- s)$. 
Now if $r\in \mathfrak{b}$ and $s\in \mathfrak{u}$, then 
$\Tr(rs)=0$. So the map 
$\mathfrak{gl}_n\longrightarrow \mathfrak{b}^*$ factors through $\mathfrak{gl}_n/\mathfrak{u}$: 
\[ 
\mathfrak{gl}_n \twoheadrightarrow \mathfrak{gl}_n/\mathfrak{u} \stackrel{\phi}{\longrightarrow} \mathfrak{b}^*. 
\] 
We claim that $\phi$ is a bijection and $B$-equivariant. 
The map $\phi$ is a bijection since if 
$\phi(\overline{s})(r)=\Tr(rs)=0$ for all $r\in \mathfrak{b}$, then $s\in \mathfrak{u}$ 
(so $\overline{s}=0+\mathfrak{u}$); so $\phi$ is injective.
For surjectivity, 
for $\Tr(r - )=t\in \mathfrak{b}^*$, it is clear that there exists $\overline{s}\in \mathfrak{gl}_n/\mathfrak{u}$ such that $\Tr(r\overline{s})=t$. 
Finally, $\phi$ is $B$-equivariant since  
$\phi(b\overline{s}b^{-1})(brb^{-1})=\Tr(r\overline{s})=\phi(\overline{s})(r)$.  
Thus, if $\mathfrak{b}$ is the space of upper triangular matrices, 
we can essentially think of $\mathfrak{b}^*$ as the space of lower triangular matrices. 
Now, from \eqref{equation:constructing-gs-resolution-g-action} and \eqref{equation:constructing-gs-resolution-b-action}, 
we have the following moment maps: 
\[ 
\begin{aligned}  
T^*(G)\cong G\times \mathfrak{g}^* \rightarrow \mathfrak{g}^*, &\hspace{4mm}(g',\theta)\mapsto \theta,  
		\hspace{6mm}
T^*(\mathbb{C}^n)\cong \mathbb{C}^n \times (\mathbb{C}^n)^*\rightarrow \mathfrak{g}^*, \hspace{4mm}(i,j)\mapsto ij, \\ 
T^*(G)\cong G\times \mathfrak{g}^*\rightarrow \mathfrak{b}^*, &\hspace{4mm}(g',\theta)\mapsto \overline{\theta},  
		\hspace{6mm}
T^*(\mathfrak{b})\cong \mathfrak{b}\times \mathfrak{b}^*\rightarrow \mathfrak{b}^*, \hspace{4mm}(r,s)\mapsto [r,s], \\ 
\end{aligned} 
\] 
where $\overline{v}:\mathfrak{g}^*\rightarrow \mathfrak{b}^*$ is a projection. 
By Propositon~\ref{proposition:group-action-on-product-space}, 
$T^*(G\times \mathfrak{b}\times \mathbb{C}^n)\rightarrow \mathfrak{g}^*\times \mathfrak{b}^*$ is the map 
\[ 
(g',\theta,r,s,i,j)\mapsto (\theta +ij, [r,s] + \overline{\theta}).  
\]  
We will explain how to obtain some of the above moment maps. 
Let $G$ act on $T^*(G)=G\times \mathfrak{g}^*\stackrel{1\times \Tr}{\cong} G\times \mathfrak{g}$ by right translation: 
$g.(g',\theta)=(g'g^{-1},g\theta g^{-1})$. 
Let $g_i$ be the coordinates of $g'$,  
$\theta_i$ be the coordinates of $\theta$, and 
let $\omega=\sum_{i} dg_i\wedge d\theta_i$ be a symplectic form on $T^*(G)$. 
Let $X=\sum_i \partial/\partial g_i$. 
Then 
\[
d\mu^X =\iota_X\omega =\sum_i d\theta_i = \omega(X). 
\] 
So $\mu^X = \sum_i\theta_i.$ 
Viewing $\theta\in \mathfrak{g}$ as a vector in $\mathbb{C}^{n^2}$, 
$\sum_i\theta_i=\theta\circ (1,\ldots, 1)$. 
Since $\mu^X(g',\theta)=\langle \mu(g',\theta),1\rangle$
where $\mu:T^*G\rightarrow \mathfrak{g}^*\stackrel{\Tr}{\cong}\mathfrak{g}$, 
$\mu(g',\theta)=\theta$. 



Suppose $G$ acts on $T^*\mathbb{C}^n$ via $g.(i,j)=(gi,jg^{-1})$.
Let $\omega=\sum_{i=1}^n dx_i\wedge dy_i$, where $(x_i)$ are the coordinates of $\mathbb{C}^n$ and $(y_i)$ are the coordinates of $(\mathbb{C}^n)^*$.
We will explicitly write down the moment map for $n=2$.
Let $X=E_{11}\in \mathfrak{gl}_2$, which is a $2\times 2$ matrix with $1$ in the $(1,1)$ entry and $0$ elsewhere. 
Since 
\[ 
\begin{aligned} 
\dfrac{d}{dt}(\exp(t 
\bordermatrix{
& &   \cr 
& 1& 0\cr 
& 0& 0\cr 
}
).(i,j))|_{t=0}
&= \left( 
\bordermatrix{
& &   \cr 
& 1& 0\cr 
& 0& 0\cr 
}
\bordermatrix{
& \cr 
& x_1\cr
& x_2\cr }, 
- \bordermatrix{
&    &    \cr 
& y_1& y_2\cr 
}
\bordermatrix{
&  &  \cr 
&1 &0 \cr 
&0 &0 \cr 
}
\right) \\ 
&= \left( 
\bordermatrix{
&    \cr 
& x_1\cr 
& 0  \cr 
}, 
\bordermatrix{
&     &  \cr 
& -y_1& 0\cr 
} 
\right) = x_1 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_1}, 
\end{aligned}
\] 
let $X= x_1 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_1}$. 
Then 
\[ 
d\mu^X =\iota_X\omega 
= (dx_1 \wedge dy_1 + dx_2\wedge dy_2 )(x_1 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_1})
=x_1dy_1+y_1dx_1
\] 
imples $\mu^X=x_1y_1$. 
So 
$\mu^X
=\langle \mu(i,j),X\rangle
=\langle \mu(i,j),E_{11}\rangle=x_1y_1$, 
and the $(1,1)$-entry of $\mu$ is $\mu(i,j)_{1,1}=x_1y_1$. 



Now let $X=E_{12}$, with $1$ in the $(1,2)$ entry and $0$ elsewhere. 
Then we have 
\[ 
\begin{aligned} 
\dfrac{d}{dt}(\exp(t 
\bordermatrix{
& &   \cr 
& 0& 1\cr 
& 0& 0\cr 
}
).(i,j))|_{t=0}
&= \left( 
\bordermatrix{
& &   \cr 
& 0& 1\cr 
& 0& 0\cr 
}
\bordermatrix{
& \cr 
& x_1\cr
& x_2\cr }, 
- \bordermatrix{
&    &    \cr 
& y_1& y_2\cr 
}
\bordermatrix{
&  &  \cr 
&0 &1 \cr 
&0 &0 \cr 
}
\right) \\ 
&= \left( 
\bordermatrix{
&    \cr 
& x_2\cr 
& 0  \cr 
}, 
\bordermatrix{
&     &      \cr 
& 0   & -y_1 \cr 
} 
\right) = x_2 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_2},   
\end{aligned}
\] 
which implies 
$d\mu^X=\iota_X\omega = (dx_1\wedge dy_1+dx_2\wedge dy_2)(x_2 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_2})=x_2dy_1+y_1dx_2$. 
Thus we obtain the Hamiltonian $\mu^X=x_2y_1$. 
% [NOTE: the $X$ be $E_{12}$ and $E_{21}$ need to be swapped! Check details.]  
Repeat the above calculation for $E_{22}$ to get 
$X= x_2 \dfrac{\partial}{\partial x_2} -y_2\dfrac{\partial}{\partial y_2}$. 
Since $d\mu^X =\iota_X\omega = x_2dy_2 +y_2dx_2$, 
$\mu^X = x_2y_2$. 
Finally, let $X=E_{21}\in \mathfrak{g}^*$ to get that the infinitesimal action is given in coordinates as 
$x_1 \dfrac{\partial}{\partial x_2} -y_2\dfrac{\partial}{\partial y_1}$. 
Then 
$d\mu^X =\iota_X\omega=x_1dy_2+y_2dx_1$ implies $\mu^X = x_1y_2$. 

Thus we get four Hamiltonian functions from $T^*(\mathbb{C}^2)\rightarrow \mathbb{C}$, which are  
$x_1y_1, x_1y_2,x_2y_1$, and $x_2y_2$. 
Since $\mu^X=\langle \mu(i,j),X\rangle$ and since $\mathfrak{g}^*\cong \mathfrak{g}$ via sending $(X,Y)$ to $\Tr(X^tY)$,  
the moment map is given as 
\[ 
\mu(i,j)=\bordermatrix{
& & \cr  
& x_1y_1& x_1y_2\cr  
& x_2y_1&x_2y_2 \cr  
} = ij. 
\] 
 
Now let $e=E_{12}$ and $f=E_{21}$. Then 
\[ 
\begin{aligned} 
[E_{12},E_{21}] &= [e,f] = ef-fe = (x_1 \dfrac{\partial}{\partial x_2} -y_2\dfrac{\partial}{\partial y_1})( x_2 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_2})
-( x_2 \dfrac{\partial}{\partial x_1} -y_1\dfrac{\partial}{\partial y_2})(x_1 \dfrac{\partial}{\partial x_2} -y_2\dfrac{\partial}{\partial y_1}) \\ 
&=  x_1 \dfrac{\partial}{\partial x_1} + y_2\dfrac{\partial}{\partial y_2}
-( x_2 \dfrac{\partial}{\partial x_2} + y_1\dfrac{\partial}{\partial y_1})=E_{11}-E_{22}. \\ 
\end{aligned}
\] 






Next, we will discuss a concept known as reduction in stages in symplectic geometry. 
Let $G\times \mathfrak{b}\times \mathbb{C}^n\stackrel{f}{\longrightarrow} G\times_B\mathfrak{b}\times \mathbb{C}^n$ 
be a principle $B$-bundle, i.e. $B$ acts freely and transitively on the fibers of $G\times \mathfrak{b}\times \mathbb{C}^n$, preserving the fibers of 
$G\times \mathfrak{b}\times \mathbb{C}^n$, i.e., 
if $y\in (G\times \mathfrak{b}\times \mathbb{C}^n)_x$ is a point in the fiber of $x$, then $b.y\in (G\times \mathfrak{b}\times \mathbb{C}^n)_x$ still lies in the fiber of $x$ for all $b\in B$. 
Thus each fiber is homeomorphic to $B$ and 
$G\times \mathfrak{b}\times \mathbb{C}^n/B\cong G\times_B \mathfrak{b}\times \mathbb{C}^n$.  
Next, note that the map $f$ has a $G$-action which commutes with the $B$-action.  
The moment map from above 
\[
T^*(G\times \mathfrak{b}\times \mathbb{C}^n) \stackrel{\mu_{G\times B}}{\longrightarrow} 
\mathfrak{g}^*\times \mathfrak{b}^*, \hspace{4mm} 
(g',\theta,r,s,i,j)\mapsto (\theta+ij,[r,s] + \overline{\theta}), 
\] 
is $G\times B$-equivariant. 
Let 
$\psi_G:T^*(G\times \mathfrak{b}\times \mathbb{C}^n)\rightarrow \mathfrak{g}^*$ and 
$\psi_B:T^*(G\times \mathfrak{b}\times \mathbb{C}^n)\rightarrow \mathfrak{b}^*$  
be the projection maps obtained from $\mu_{G\times B}$.  
Consider $\psi_B^{-1}(0)\subseteq T^*(G\times \mathfrak{b}\times \mathbb{C}^n)$.  
Since $B$ acts freely on $\psi_B^{-1}(0)$,  
\[  
\psi_B^{-1}(0)/B\cong T^*(G\times \mathfrak{b}\times \mathbb{C}^n/B)\simeq T^*(G\times_B\mathfrak{b}\times \mathbb{C}^n) 
\]  
is a reduced space.  

Now consider $G$ acting on $\psi_B^{-1}(0)$, 
which commutes with the $B$-action. Since $G$ preserves the symplectic form, say $\omega$, 
on $T^*(G\times \mathfrak{b}\times \mathbb{C}^n)$, 
$G$ acts symplectically on the reduced space $(\psi_B^{-1}(0)/B,\omega')$, where $\omega'$ is the symplectic form on $\psi_B^{-1}(0)/B$. 
Since $B$ preserves $\psi_G:T^*(G\times \mathfrak{b}\times \mathbb{C}^n)\longrightarrow \mathfrak{g}^*$, 
$B$ preserves 
$\psi_G\circ \iota_1:\psi_B^{-1}(0)\rightarrow \mathfrak{g}^*$. 
So $\psi_G\circ \iota_1$ is constant on fibers of 
$\psi_B^{-1}(0)\stackrel{p_1}{\longrightarrow}\psi_B^{-1}(0)/B$. 
Thus, there exists a smooth map 
\[ 
\mu_G:\psi_B^{-1}(0)/B\simeq T^*(G\times_B\mathfrak{b}\times \mathbb{C}^n)\longrightarrow \mathfrak{g}^* 
\] 
such that 
$\mu_G\circ p_1=\psi_G\circ \iota_1:\psi_B^{-1}(0)\longrightarrow \mathfrak{g}^*$. 

\begin{proposition}
\mbox{} 
\begin{enumerate}
\item $\mu_G:T^*(G\times_B\mathfrak{b}\times \mathbb{C}^n)\rightarrow \mathfrak{g}^*$ is a moment map for $G$ acting on $(T^*(G\times_B\mathfrak{b}\times \mathbb{C}^n), \omega')$. 
\item Since $G$ acts freely on $\mu_{G\times B}^{-1}(0)$, $G$ acts freely on $\mu_G^{-1}(0)$ and a symplectomorphism 
$\mu_G^{-1}(0)/G\cong \mu_{G\times B}^{-1}(0)/G\times B$ exists. 
\end{enumerate}
\end{proposition}



Now, consider the reduction of $T^*(G\times \mathfrak{b}\times \mathbb{C}^n)$ by $G$ first: 
\[ 
\psi_G^{-1}(0)
= \{(g',\theta,r,s,i,j)\in T^*(G\times \mathfrak{b}\times \mathbb{C}^n):\theta+ij=0\} 
= \{(g',-ij,r,s,i,j)\in T^*(G\times \mathfrak{b}\times \mathbb{C}^n) \}.  
\] 
Since the $G$-action is transitive, we will identify 
\[ 
T^*(\mathfrak{b}\times \mathbb{C}^n) 
\cong \{(1,-ij,r,s,i,j)\in T^*(G\times \mathfrak{b}\times \mathbb{C}^n)\}\simeq \psi_G^{-1}(0)/G.  
\] 
As above, 
$\mu_B:T^*(\mathfrak{b}\times \mathbb{C}^n)\longrightarrow\mathfrak{b}^*$ is a moment map for $B$ acting on 
$(T^*(\mathfrak{b}\times \mathbb{C}^n),\omega_B)$, where $\omega_B$ is the symplectic form on $T^*(\mathfrak{b}\times \mathbb{C}^n)$. 
Secondly, since $B$ acts freely on 
$\mu_{G\times B}^{-1}(0)$, $B$ acts freely on $\mu_B^{-1}(0)$ and we have 
\[ 
\mu_B^{-1}(0)/B \cong \mu_{G\times B}^{-1}(0)/G\times B. 
\] 

Thus studying the $G$-orbits on $T^*(G\times_B \mathfrak{b}\times \mathbb{C}^n)$ is equivalent to studying the $B$-orbits on $T^*(\mathfrak{b}\times \mathbb{C}^n)$. 
A discussion of the Hamiltonian reduction is also given in \cite{Nevins-GSresolutions}.  

 

 

Now, let $B$ be the set of invertible upper triangular matrices and let $\mathfrak{b}=\lie(B)$. The adjoint action of $B$ on $\mathfrak{b}\times \mathbb{C}^n$ is $b.(r,i)=(brb^{-1},bi)$, which is induced onto 
$T^*(\mathfrak{b\times \mathbb{C}^n})$ via $b.(r,s,i,j)=(brb^{-1},bsb^{-1},bi,jb^{-1})$. 
In terms of Section~\ref{subsection:filtered-quiver-varieties}, we will explain how $T^*(\mathfrak{b}\times \mathbb{C}^n)$ is identified as the cotangent bundle of filtered quiver variety. 

Let $Q$ be the $1$-Jordan quiver $\xymatrix@-1pc{\stackrel{1}{\bullet}\ar@(ur,dr)^a}$ 
and let $\beta=n$.  
Let $F^{\bullet}$ be the complete standard filtration of vector spaces of $\mathbb{C}^n$. 
Then  $F^{\bullet}Rep(Q,n)=\mathfrak{b}$. 
Now we adjoin a framing to the $1$-Jordan quiver to get 
$Q^{\dagger}: \xymatrix@-1pc{ \stackrel{1^{\natural}}{\circ}\ar[rr]^{\iota_1} & & \stackrel{1}{\bullet}\ar@(ur,dr)^a }$.  
Let $\beta^{\dagger}=(n,1)$ where $F^{\bullet}$ is imposed only on the representation at the nonframed vertex. 
This gives us a $B$-action on 
$F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger})\cong \mathfrak{b}\times \mathbb{C}^n$.  
One doubles this quiver $Q^{\dagger}$ to obtain 
\[ 
\xymatrix@-1pc{
\stackrel{1^{\natural}}{\circ} \ar@/^/[rrr]^{\iota_1} & & & \stackrel{1}{\bullet} \ar@/^/[lll]^{\iota_1^{op}} \ar@(ul,ur)^{a} \ar@(dr,dl)^{a^{op}}  \\ 
}
\] 
and we have the identification  
$T^*(F^{\bullet}Rep(Q^{\dagger},\beta^{\dagger}))\cong 
T^*(\mathfrak{b}\times \mathbb{C}^n)$. 
%\[ 
%\xymatrix{ 
%\stackrel{1}{\bullet} \ar@(l,d)[]_{r}  \ar@(l,u)[]^{s}  \ar@/^/[rr]| j 
%&& \stackrel{2}{\circ} \ar@/^/[ll]|{i}
%} 
%\]

 


%DELETE BELOW. 
%
% 
%Consider $B$ acting on $\mathfrak{b}\times \mathbb{C}^n$ via the adjoint action $b.(r,i) %= (brb^{-1},bi)$. 
%Then consider $T^*(\mathfrak{b}\times \mathbb{C}^n)=\mathfrak{b}\times \mathfrak{b}^*\times \mathbb{C}^n\times (\mathbb{C}^n)^*$. Here, we explain $\mathfrak{b}^*$: consider the map 
%\[  \mathfrak{gl}_n \stackrel{\psi}{\longrightarrow} \mathfrak{b}^* = \Hom(\mathfrak{b},\mathbb{C}), \hspace{4mm} 
%r\mapsto (s\mapsto \Tr(rs)).  
%\]  
%Consider $r\in \mathfrak{n}_+$, which is the set of strictly upper triangular matrices in $\mathfrak{gl}_n$. Then for $s\in \mathfrak{b}$, we have $\Tr(rs)=\Tr(sr)=0$. 
%This implies that $\ker \psi = \mathfrak{n}_+$ and 
%$\psi$ factors through $\mathfrak{gl}_n/\mathfrak{n}_+$: 
%\[ 
%\xymatrix@-1pc{ 
%\mathfrak{gl}_n \ar[rrrr]^{\psi} \ar[drdr] & & & & \mathfrak{b}^* \\ 
%		& &				 & &  \\  
%& & \mathfrak{gl}_n/\mathfrak{n}_+ \ar[uurr] & & \\   
%} 
%\]  and thus $\mathfrak{b}^*$ may be identified with $\mathfrak{gl}_n/\mathfrak{n}_+$, %i.e., one can think of $\mathfrak{b}^*$ as the set of lower triangular matrices. 

  









 
